Characterizing Stage-Aware Writing Assistance in Collaborative Document Authoring

Writing is a complex non-linear process that begins with a mental model of intent, and progresses through an outline of ideas, to words on paper (and their subsequent refinement). Despite past research in understanding writing, Web-scale consumer and enterprise collaborative digital writing environments are yet to greatly benefit from intelligent systems that understand the stages of document evolution, providing opportune assistance based on authors' situated actions and context. In this paper, we present three studies that explore temporal stages of document authoring. We first survey information workers at a large technology company about their writing habits and preferences, concluding that writers do in fact conceptually progress through several distinct phases while authoring documents. We also explore, qualitatively, how writing stages are linked to document lifespan. We supplement these qualitative findings with an analysis of the longitudinal user interaction logs of a popular digital writing platform over several million documents. Finally, as a first step towards facilitating an intelligent digital writing assistant, we conduct a preliminary investigation into the utility of user interaction log data for predicting the temporal stage of a document. Our results support the benefit of tools tailored to writing stages, identify primary tasks associated with these stages, and show that it is possible to predict stages from anonymous interaction logs. Together, these results argue for the benefit and feasibility of more tailored digital writing assistance.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.


==> sec.Methodology.tex <==
\section{Stage-Aware Writing Assistance}
\label{methodology}

Our work is motivated by two connected research questions. First, we wish to understand, cognitively, how and whether authors perceive that there are stages in their writing process.  Second, we wish to explore how user actions vary over a document's editing lifespan.  As we note earlier in the paper, while others have explored the stages of writing, many past studies seem focused either with respect to domain -- documents of a certain type -- or sample size.  

To address these two questions, we studied the stage of a document and how it captures the situated writing assistance using two complementary methodologies: (1) a survey of information workers at a large technology company, and (2) a large-scale log analysis of a popular digital writing platform over several million documents. In this section, because of the connected and complementary nature of the study, we describe the methodology for both of these studies: our survey and our log analysis.

\begin{comment}
Our main research question is to investigate whether providing writing assistance that is tailored to the current stage of a document development is beneficial to the writers of that document, both in individual and collaborative settings.
To this end we need to better characterize two different aspects of \textit{stage-aware writing assistance}: 
\begin{enumerate}
    \item \textbf{Characterizing the stage of a document:} How are the stages of document evolution perceived by the writers?
    \item \textbf{Characterizing stage-appropriate writing assistance:} \\What writing assistance is beneficial at different stages of document evolution?
\end{enumerate}

To address these two questions, we studied the stage of a document and how it captures the situated writing assistance using three complementary techniques: a survey of information workers at a large technology company, a large-scale log analysis of a popular digital writing platform over several million documents as well as a preliminary investigation into the utility of user interaction log data for predicting the temporal stage of a document. 

While the log analysis provides valuable information about general patterns in users interactions with a digital writing environment, a qualitative analysis of our survey responses resulted in a distinct characterization of stages of document authoring based on authors' conceptual models of this process which was not possible to study using log analysis. 

In this section, we describe these data sources as well as the main steps to the analysis of both qualitative and quantitative data.
\end{comment}

\subsection{Survey}
\label{Survey}
Our survey was motivated by a desire to investigate whether providing writing assistance that is tailored to the current stage of a document under development is beneficial to the writers of that document.
To this end, we need to better characterize two different aspects of \textit{stage-aware writing assistance}: 
\begin{enumerate}
    \item \textbf{Characterizing the stage of a document:} How are the stages of document evolution perceived by the writers?
    \item \textbf{Characterizing stage-appropriate writing assistance:} \\What writing assistance is beneficial at different stages of document evolution?
\end{enumerate}

To elicit people's perspectives on writing stages and whether stage-appropriate assistance might be beneficial, we distributed a survey within a large technology company. The survey included both closed and open-ended questions. We collected 183 completed responses to this survey (response rate: 10\%, completion rate: 74\%). 
% From an email list of \el{number of employees on list}, we collected 175 complete or partial responses to our survey.  The completion rate of the survey from these 175 responses was 70\%.\bs{add response rate} 
% survey at a large technology company with a range of close-ended as well as open-ended questions. The survey data helped us understand how enterprise workers approach the writing of a document, how the stages of document authoring are perceived by them and their expectations for types of writing assistance at these stages.

Our survey started with a section on demographics including job roles, number of current projects, and team size. The next section involved different questions regarding writing documents at the workplace. These questions helped us verify whether writing documents at the workplace is a common practice, what tools are frequently used for writing documents, and how often these documents involve other collaborators.
Finally, the main segment of our survey asked participants to reflect on their perception of the utility of an intelligent writing assistant and how stage-aware writing assistance should be realized.

Respondents came from a diverse set of roles ranging from product managers and software developers to sales people and administrative assistants, the majority had been working at the company for more than 5 years (63\%).  Multi-tasking on different projects was a common trend among them, with 75\% working on at least 3 projects in parallel at the time of completing the survey.

\subsubsection{Analysis.}
The responses to close-ended questions were aggregated to provide general statistics on participant demographics and writing habits.  

The responses to open-ended questions were analyzed using affinity diagramming. Data was initially clustered using open coding \cite{corbin1990grounded} producing
19 clusters. Clusters were then analyzed using axial coding \cite{corbin1990grounded} to identify overall themes in the data.  We found that saturation for our
qualitative data occurred approximately after 80 participants, and from this point no
new clusters of information were identified. However, we continued
to cluster responses for the remaining participants, particularly
attuned to data that might expand our clusters or add nuance to
our analysis. 

\subsection{Log Data Analysis}
\label{LogDataAnalysis}
We analyzed a sample of the anonymous interaction logs from users of a major Web-scale commercial writing application\footnote{name suppressed for blind reviewing} over a three-month period from February 1 to April 30, 2019. 

To create this dataset, we collected a subset of document candidates in English from the US market that were created within a 2 week period from February 1 to February 15. For these documents we collected logs of user interactions with different functionalities available through the application UI.\footnote{This modern, widely used word processing application provides standard functionalities including copy-paste, formatting, commenting, change tracking, etc.}
Our sample consists of approximately 16 million document candidates and approximately 16.6 million unique writers who accessed these documents.

To safeguard the private data of our writers, we leveraged interaction logs devoid of textual data and writer data. The only exception to this was a system generated ID assigned to an individual writer that served to uniquely map the set of interactions of that writer on a document. These interaction logs are highly granular and include approximately 2000 unique commands. For a subset of these documents, we generated numeric statistics on document content (e.g., \texttt{\#}words,  \texttt{\#}sentences,  \texttt{\#}charts, etc), logged as static snapshots at different time points.
Finally, for an even smaller subset of documents, we have access to some statistics on typing traces that includes timing information on the duration of typing by different users with respect to a document. We do not have access to keystroke-level data or the actual characters that were typed.

\begin{comment}
Our interaction logs contain neither any textual data, nor any information about the users besides a system generated ID that can be used to uniquely map the set of interactions on a document to the corresponding user. These interaction logs are very granular and include roughly 2000 unique commands.
%\rw{I'd be clear here that the logs are really granular - command level}
For a subset of these documents, we also have some numeric statistics on their content (e.g.,  \texttt{\#}words,  \texttt{\#}sentences,  \texttt{\#}charts, etc) that are logged as static snapshots at different time points.
Finally, for a yet smaller subset of documents, we have access to some statistics on typing traces that includes timing information on the duration of typing by different users with respect to a document. We do not have access to any keystroke-level data or the actual characters that were typed.
\end{comment}
%\vspace{-2mm}
\begin{figure}[htb]
\centering
\includegraphics[width=0.80\textwidth]{Lifetime_vs_numCollabs.png}
\caption{Distribution of average document lifetime across different number of collaborators.}
\label{Lifetime_vs_numUsers}
\end{figure}
%\vspace{-1mm}
\subsubsection{Lifetime of Documents}
Since the stage of a document evolution is closely related to its lifetime, we 
%For our purposes, the lifetime of a document ranges 
defined the document lifetime as the time interval from its creation to the last user interaction with the document during our three-month window.%\rw{Reflecting on this a bit - we're a lot less likely to see documents in the range 61-90 because they would have to be started near the beginning of the 3-month window. I wonder what impact this has, if any, on our analysis}
We find that the majority of documents in our collection have a short lifetime (less than 24 hours - See Figure \ref{LifetimeDist} - gold/left).  
In addition, there is a correlation between the number of collaborators involved in a document and the lifetime of the document. Figure \ref{Lifetime_vs_numUsers} shows that the lifetime of documents has a non-decreasing trend as the number of authors increases ($r = 0.78, n = 20, p < 0.0001$). 
%\bs{Pearson correlation statistics based on documents up to 20 users.}

\begin{comment}
\begin{figure}[htb!]
\centering
\includegraphics[width=0.5\textwidth]{LifetimeDist.png}
\caption{Distribution of average document lifetime across different number of collaborators. Documents with lifetime shorter than 1 hour are removed.} 
%\rw{why? can we say anything about the frequency of those? why they might have such a short lifetime?}.}
\label{LifetimeDist}
\end{figure}
\end{comment}
%\vspace{-1mm}

\subsubsection{Pre-processing} \label{FinalDataSet}
We take two pre-processing steps to address limitations in our log data and prepare it for more robust analysis. 
Firstly, logged interactions are at a very fine-grained command level: we have over 2000 unique commands in our logs, each of which can be relatively sparse in its occurrence. 
%In the first step we
%address two limitations with our logs: (1) Our dataset does not include any information on the content of documents and textual changes beyond a fine-grained set of commands capturing users' interactions with the writing application; and (2) these logged interactions are at a very fine-grained command level: we have over 2000 unique commands in our logs, each of which can be relatively sparse in its occurrence. 
To address this, we need to provide a mapping between low level user actions to higher level activities, which are interpretable and correspond to meaningful writing behavior.
To develop initial categories of activities, a subset of all commands were reviewed by three annotators independently to identify the impact of applying those commands to the writing environment. The impact of a command was investigated based on widely accepted operations that change the content of a document (i.e., adding, editing, and deleting) as well as commands that have no impact on the document content (e.g., viewing, navigating, communicating, etc).

%\vspace{-1.5mm}
\begin{figure}[htb!]
\centering
\includegraphics[width=0.80\textwidth]{LifetimeDist_Combined.png}
\caption{Distributions of document lifetime before (gold - left) and after (blue - right) pre-processing} 
\label{LifetimeDist}
\end{figure}
%\vspace{-1mm)

The annotators then engaged in an iterative vetting and refining process %\footnote{Iterative vetting involves using the output of one stage to determine the next stage, incrementally reaching a final objective.}
to group commands based on how they impact the document and the writing environment. %in general and refined the formed groups until no more groups were found.
For example, all commands that result in adding some content (text, shapes, citations, etc.) to the document are grouped together as \textit{Adding}, while commands that are only used for navigating throughout the document (e.g., NextHeader, GoToPreviousPage, etc.) are grouped into the \textit{Navigation} activity.
Annotator agreement was moderate, at 67\% majority agreement between the three annotators.
%Since there is not much ambiguity in whether a specific command impacts the document content the agreement among the annotators was generally high with 67\% observed agreement across the three annotators. %\rw{reviewers are going to want to see a number for kappa or at least \% agreement}. 

These sets of activity groups were then unified by resolving conflicts across annotators and finalizing a repository of activity categories. Finally, one of the annotators completed the groupings for the remaining commands based on this repository.
%As a result, a taxonomy of 48 activity categories was created.
This resulted in a set of 48 activity labels. These activity labels were then classified into 11 higher level activity categories that more closely correspond to writing activities. Figure \ref{CategorizingCommands} shows a subset of the higher levels of this taxonomy. These high level groupings are sufficiently general and are supported by many modern writing tools.

\begin{figure}[htb]
\centering
\includegraphics[width=0.80\textwidth]{commands_BW.pdf}
\caption{Taxonomy of writing commands in our dataset. Note that only the top two levels are shown.}
\label{CategorizingCommands}
\end{figure}

% \bs{The following paragraph was written based on our attempt to justify why we are only considering multi-author docs in most of our analysis. I suggest we just replace it with explicitly mentioning our aim for understanding CW scenarios, while in essence, our methodology applies to SAW as well + SAW can be considered a simplified version of CW process. Any thoughts?}
% The second pre-processing step is used to tease out the different roles that writers adopt through stages of writing. While writers in individually authored documents do assume different roles as they progress through writing a document, we hypothesize that these roles are likely to stand out more clearly when multiple authors write collaboratively. 

The second pre-processing step is used to filter out all documents with a single author throughout their lifetime. While writers in individually authored documents do progress through a similar yet simplified subset of writing activities (as characterized by Lowry et al. \cite{lowry2004}), we are focused on characterizing stages of document evolution where multiple authors write collaboratively.  
Thus we limit most of our analyses to documents that log interactions from 2 to 10 users\footnote{Our survey confirms (see Section~\ref{sec:qualfind}) that 98\% of collaboratively authored documents have no more than 10 users.}. Note that our methodology is, in general, agnostic to the number of users, and
throughout the rest of the paper we will show some results that equally apply to individually authored documents.

Finally, in order to reduce noise in the dataset, we eliminate documents that have a lifetime shorter than 1 hour.
%The second step of our preprocessing involved a principled way of reducing noise in our collection of documents by removing documents with very short lifetimes that do not provide enough interaction signals for studying document authoring behavior. To this end, we limited our analysis to documents with at least 2 users as they tend to correlate with longer lifetimes. \rw{we need to be very careful in how we justify this - it has implications for the generalizability of the findings} Further, we used 10 users as an upper bound since our survey data indicated that 98\% of shared documents that are written for work purposes involve between 2 and 10 collaborators.  Finally, all documents with lifetime shorter
%than 1 hour were removed from the dataset as they won’t represent
%meaningful writing scenarios.
%\subsubsection{Final Dataset}
%\label{FinalDataSet}
Our final dataset comprises approximately 170k documents where the majority has 2 or 3 collaborators involved (78\% and 12\% respectively). The lifetime of documents in this final set are higher and more evenly distributed overall (Figure \ref{LifetimeDist} - blue/right).
%\vspace{-1mm}
\begin{comment}
\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{LifetimeDist_CW.png}
\caption{Lifetime of collaborative documents in the preprocessed dataset.}
\label{LifetimeDist_CW}
\end{figure}
%\vspace{-1mm}
\end{comment}





==> sec.QualitativeAnalysis.tex <==
\section{Stage-aware Writing Assistance} 
Our main research question is to investigate whether providing writing assistance that is tailored to the current stage of a document development is beneficial to the writers of that document.
To this end we need to better characterize two different aspects of \textit{stage-aware writing assistance}: 
\begin{enumerate}
    \item \texttt{Characterizing the Stage of a Document:} How are the stages of document evolution perceived by the writers?
    \item \texttt{Characterizing the Writing Assistance:} What writing assistance is beneficial at different stages of document evolution?
\end{enumerate}

% There are many open questions in this space including how common writing documents at the workplace is, what support is needed, what are the expectations of an intelligent writing tool and whether there is a need for tailored support at different stages of writing?

To address these two questions, we began by conducting a survey at a large technology company with a range of close-ended as well as open-ended questions. 
% Most research on the writing process has been carried out in the context of education. Thus, little focus has been put on the particularities which arise when the writing process is carried out by information workers who need to write documents as a part of their daily routine at the workplace.
The survey data helped us understand how enterprise workers approach the writing of a document, how the stages of document authoring are perceived by them and what the expectations are for types of writing assistance at these stages.

\subsection{Survey}
We distributed a survey within a large technology company and collected 175 responses (completion rate: 70\%). 
Our survey started with a section on demographics including Job roles, number of current projects, team size, etc. The next section involved different questions regarding writing documents at the workplace which helped us verify whether writing documents at the workplace is a common practice, what tools are frequently used for writing documents and how often these documents involve other collaborators as well.

Respondents came from a diverse set of roles ranging from product managers and software developers to sales people and administrative assistants, the majority have been working at this company for more than 5 years (63\%).  Multi-tasking on different projects was a common trend among them, with 75\% working on at least 3 projects.
\subsection{General Findings}
%Our survey data confirmed that writing documents is very common at the workplace. 
87\% of our respondents mentioned they do need to write documents as a part of their work routine. They use a wide range of writing tools including Microsoft Word Desktop Client (89\%) and Online Client (49\%), followed by Notepad / Notepad++ (19.3\%), OneNote (16\%), Overleaf / Sharelatex (11.1\%), Google Docs (8.2\%), etc.

Collaboration on these documents was also a common theme among our participants with the majority (74\%) collaborating on at least 25\% of their documents.
Despite the commonality of collaborative writing, a closer examination of the qualitative responses (discussed below) indicated that the need for tailored support in different stages of document authoring is associated with both Single Author Writing (SAW) and Collaborative Writing (CW) scenarios. 
%While some of the participants talked about multi-author scenarios, the majority of responses could be applied to either of these scenarios. 
% Single author Writing (SAW) is defined as writing conducted by one individual that involves planning, drafting and reviewing (Lowry et al., 2004) Collaborative Writing (CW) builds on single-author writing by involving multiple people, thus increasing the complexity of the writing process (Galegher and Kraut, 1994).
\begin{quote}
\textit{``in and ideal scenario I would just do some sort of content dump to the system and the system structures this text. So that I don't have to think about paragraphs, sections, where to put what etc. And then in later stages I want help with how to nicely formulate things. That's not only in a collaborative setting though.''} [P10]
\end{quote}
As a first step towards understanding whether or not there is a need for different types of support at different stages of document evolution, in the next segment of our survey 
%included a series of questions to gauge real users perceptions and attitudes towards this concept. More formally, 
the participants were asked \textit{``Should an intelligent writing assistant provide different types of support at different stages of writing in the document?''} with a binary Yes / No response type.

Over 70\% of our participants expressed a need for different types of support at different stages of writing. The follow up open-ended questions to elaborate on their rationales for their response to this initial question revealed how these stages are perceived by the participants and that what support is needed at these stages. 

The responses to these questions were all analyzed using affinity diagramming. Data was initially clustered using open coding producing
19 clusters. Clusters were then analyzed using axial coding to identify overall themes in the data. We found that saturation for our
qualitative data occurred approximately after 80 participants, no
new clusters of information were identified. However, we continued
to cluster these responses for the remaining participants, particularly
attuned to data that might expand our clusters or add nuance to
our analysis. These clusters resulted in four broad themes, corresponding to different notions of the stage of a document as perceived by our participants and the utility of different types of writing assistance based on these stages.

The following three subsections elaborate on three different perceptions of a document's stage and the final subsection describes a different implication of awareness of the stage of a document that is essential for more effective collaboration over writing documents.

% (1) Supporting Early versus Later Stages of Document Evolution; (2) Supporting different phases of writing; (3) Supporting different modes or intents of writing; and (4) Awareness of Stage of Document is essential both for the intelligent System and the collaborating writers. We describe more details about these themes in the following subsections.

% better characterization of the

\begin{comment}
\subsection{Stage-based Support for both SAW and CW}
%Writers require different support at different stages of writing both in SAW and CW scenarios.

Single author Writing (SAW) is defined as writing conducted by one individual that involves planning, drafting and reviewing (Lowry et al., 2004)
Collaborative Writing (CW) involves multiple people, thus increasing the complexity of the writing process (Galegher and Kraut, 1994).

%While the complexity of CW scenarios is generally more amplified relative to SAW scenarios, 
A qualitative analysis of these survey responses indicated that the need for tailored support at different stages of writing is not only desirable for CW settings: the majority of responses are applicable to either of these scenarios. 
\begin{quote}
\textit{``in and ideal scenario I would just do some sort of content dump to the system and the system structures this text. So that I don't have to think about paragraphs, sections, where to put what etc. And then in later stages I want help with how to nicely formulate things. That's not only in a collaborative setting though.''} [P10]
\end{quote}

In unpacking the quote above we also see a time-based notion of stages of document writing that is further discussed in the following subsection.
\end{comment}

\subsection{Temporal Stages of Document Authoring}
The Stages Model of Writing \cite{rohman1965} focuses on the evolution of the text as an external by-product of the writing where the main three stages of pre-writing, writing and rewriting are separated in time. 
% While more recent models (e.g. Flower and Hayes's model \cite{flower1984}) argue that a more realistic model of writing needs to focus on the mental processes involved in the writing process and that these mental processes are interleaved, hierarchically embedded and are not executed in a linear order, these models are indeed complementary and are not in conflict (Mitchell, 1996). 

%In fact, once we shift our view to the document as the by product of this process we can see some time based ordering of these high level stages of document evolution. 

This time-based ordering of document stages was shared amongst many of our participants who referred to them as early versus later stages of document writing. The qualitative analysis of their description of these early and late stages resulted in a novel characterization of these temporal stages, which high level writing phases and low level writing activities are associated with them, and which types of writing assistance are appreciated in each stage and what support is perceived as interruption.

Our participants perceived the early stages of writing to be highly focused and many participants expressed a desire for fewer interruptions and fewer system suggestions and notifications during these stages, particularly about minor fixes and improvements. 

%\advance\leftmargini 0.05em
\begin{myquote}{0.2in}
\textit{``I want fewer interruptions when i am focusing on adding content early in the document writing process.''} [P11]\\
\textit{``As someone who primarily writes documents in LaTeX, I like the ability to focus on writing the content without having to worry about formatting. Then only once the content is put down do I go back and tweak the look of the document. This allows me to focus on different aspects of the documents at different stages.''} [P12]\\
\textit{``Notifying me of grammar and spelling errors when I'm trying to get my thoughts out is really just a distraction. I prefer when these suggestions are made at a later editing stage.''} [P40]
\end{myquote}
The qualitative analysis of these responses indicated that participants can associate different phases of writing including Planning, Outlining and Early Drafting to \textit{Early Stages of Writing}. 

As well, participants discussed a variety of activities in earlier stages of writing which revealed the types of support that are the most appreciated in these early stages. Among them, outlining and deciding on the structure of the document as well as searching for relevant content were perceived as early stage activities. 
\begin{myquote}{0.2in}
    \textit{``Brainstorming and scope defining support \textbf{early on} that helps develop a basic outline and framework. It would be great for a writing assistant to help with the `starting from nothing' phase.''} [P98]\\
    \textit{``The needs at different stages may be very different. E.g. for structural changes, they better take place as \textbf{early} as possible; while for minor fixes or suggestions, they can come \textbf{later} when the body of text is by and large stable.''} [P64]\\
    %\textit{``When \textbf{getting started}, Outline or Structure help is needed; \textbf{Later on} in the process, Editing, fact checking, adding references type of help is needed.''} [P84]\\\\
    %\textit{``\textbf{Early:} Focus and scope - needed at the beginning to understand what to write about and how much; this is often org dependent and the ability to create org-specific templates and help advice would be amazing.  \textbf{Mid:} Content analysis and comparison, to highlight style and completeness differences in different areas.  \textbf{Late:} Advice on structural features and cleanups that can save time and improve accessibility.''} [P219]\\\\
    \textit{``Would be great to enter some notes and have an outline constructed. \textbf{Later} it would be great to have research done for me if I need a supporting quote or need a chart from another document. \textbf{Finally} it would help to have suggestions for alternatives to overused words.''} [P57]
\end{myquote}
Similarly, participants described a variety of activities that are not crucial to earlier stages of writing, for those activities system support can be perceived as \textit{distracting}, \textit{annoying} or \textit{not necessary}.
Overall, minor fixes, proofing and grammar fixes, collaborative activities such as commenting and change tracking are perceived as not helpful nor appreciated during early stages of document evolution.
\begin{myquote}{0.2in}
    \textit{``Different actions and needs are required for each stage of writing; i.e. there is no need to suggest spacing and layout changes when I've just started writing down my thoughts (the text is "under-construction" and liable to change quickly).''} [P70]\\
    \textit{``Worrying about complete sentences and grammar while brainstorming would slow things down considerably ... but necessary for a final release.''} [P227]\\
    \textit{``Initial document writing is mainly non-collaborative, whereas later it's a matter of tweaking and improving with the feedback of others.''} [P178]
\end{myquote}
Later stages, on the other hand, are described as the time when most of the content has been added to the document and the writers can now focus on improving different aspects of the document during Reviewing and Copy-Editing phases.

\begin{myquote}{0.2in}
    \textit{``Document creation and document perfection are fundamentally different.  In my opinion, the best way to create a collaborative document is to get a rough draft made as quickly and dirtily as possible and then begin to improve it; different forms of assistance are required for each scenario.''} [P237]\\
\end{myquote}

Another interesting quality of later stages is that the document is known to be more ``mature'' with most of the content already included and structured. This quality has at least two different implications for what support can and should be provided at earlier versus later stages of writing. First, since in later stages the structure and the content of the document is highly stable the system can provide more end to end and global feedback as opposed to suggestions that are relevant to a specific part of the text only (e.g. identifying missing topics to be included versus spelling errors to be fixed). Second, with more content in place and a longer history of edits, intelligent writing assistants can be more reliable in predicting what support is needed.  

\begin{myquote}{0.2in}
    \textit{``When I'm actively working on creating the document I want suggestions around better writing style, but focused on what I'm doing at that moment.  Once the document is more mature I'd want feedback on the end to end document, not a specific word here or there.''} [P106]\\
    \textit{``During the draft phase, there will be a lot of changes that just won't stick. At reviewing phase it would be helpful to objectively view the whole document to suggest improvements.''} [P207]\\
    %\textit{``Once a lot of content is in a document, a `bot' may be able to warn that you are going to change something that was just edited.''} [P77]\\\\
    \textit{``Intelligence should improve as the document matures.  The intent of the document, the subject matter, and the style of the document will become more clear as it evolves.''} [P78]
\end{myquote}

Given that the main focus of later stages is on improving the document, different later stage activities are identified as Proofreading e.g. proofing and formatting, Task Management (e.g. addressing pending comments or TODO items), Collaborative Activities such as adding collaborators, communicating with collaborators through comments and change tracking functionalities, etc. as well as Reviewing and Finalizing activities including fact checking, adding references, setting required permissions, etc.

\begin{myquote}{0.2in}
    \textit{``When getting started, Outline or Structure help is needed Later on in the process, Editing, fact checking, adding references type of help is needed ''} [P84]\\
    %\textit{``[In later stages] 1. Update me of unaddressed/unread comments that I should follow up on. 2. Help me identify similar comment available in other documents that I can use for reference.''} [P37]\\\\
    \textit{``At the drafting stage, making sure the document is structured properly and all the bases are covered is paramount. At later stages, getting feedback and sign-off become much more important. It'd be great to more easily track changes.''} [P154]\\
    \textit{``At the end of the writing process it is helpful to have a spelling and grammar check, with perhaps some suggestions on structure, yet I find suggestion DURING writing to be distracting.''} [P182]
   % \textit{``At the beginning providing table contents, title formats, and captioning. Later can add references, etc.''} [P194]\\
\end{myquote}

%The main takeaways from what was discussed can be summarized as three implications for design:
The following three design implications are our main takeaway from the preceding analysis:
\begin{enumerate}
    \item Intelligent Support should be provided based on the activities that are pertaining to the current stage of document evolution (i.e. early versus later stages).% in order to be appreciated by the writers.
    \item Writers are in a focused mode during earlier stage of writing and the interruptions by the system should be minimized. 
    \item Users can benefit from a higher level of control over the writing process in earlier stages with outlining, structuring or searching functionalities that are provided on demand. During later stages intelligent systems can be more proactive in providing feedback and suggestions to improve the overall document quality.
\end{enumerate}

\subsection{Phases of Writing}
% According to Lowry et al's Taxonomy of Writing Activities \cite{lowry2004}, 
Different models of writing process \cite{flower1984, lowry2004} state that writers go through different phases throughout the document authoring process. These phases are characterized as brainstorming, outlining, drafting, reviewing, revising and copy editing \cite{lowry2004} or more broadly as planning, translating and reviewing \cite{flower1984}. 
%This view of writing activities is largely inline with Flower and Hayes model that specifies planning, translating and reviewing as three main processes involved.

A qualitative analysis of our participants' responses reveals that the idea of going through different phases of writing during the process of writing documents resonates with them and that they perceive the stage of the document based on these phases of writing. In fact these phases were described in a variety of terms:
\textit{``from document creation to document perfection''} [P237], \textit{``starting from nothing phase''} [P98], \textit{``Rough draft vs final draft''} [P?], \textit{``Draft, Editing, Polishing''} [P?, P220], \textit{``Creative or Brainstorming, `culling the first main draft', draft editing, reviewing, finalizing''} [P?] \textit{``Outlining, Writing, Consulting''} [P158], \textit{``Schedule (content requirements), Reminders \& goals, Refresh''} [P135], \textit{``early drafting, end of drafting, reviewing''} [P224] etc.

%Similar to the theme described in the previous subsection those participants who resonated with these phases of writing
% Participants described groups of activities that are associated with each phase and hence could use targeted support during that phase.
In probing the ways our participants described these phases of writing we noted an overarching temporal ordering to these phases as well as a variety of activities that are associated with each phase.

\begin{myquote}{0.2in}
    \textit{``There are appropriate tasks for every phase that might not apply for all others and assistance in remembering them would be great. Like assistance for spellcheck/alignment  is much better suited to the end of \textbf{drafting}. Reminders to share or tag people are better suited for \textbf{reviewing}.''} [P224]\\
    \textit{``Different stages require different approaches: \textbf{drafting} is a ``throw in all ideas'', but \textbf{finalizing} is ``polish wording and structure''.  E.g.: Worrying about complete sentences and grammar while brainstorming would slow things down considerably … but necessary for a final release.''} [P227]\\
    %\textit{``\textbf{Brainstorming} vs. \textbf{Authoring} vs. \textbf{Finalizing} have very different needs.''} [P138]\\\\
    \textit{``Writing stages differ: \textbf{Creative or brainstorming}. Culling the main \textbf{first draft}. \textbf{Draft editing} and \textbf{review}. \textbf{Finalization} of the document. Each involves a different skill set.''} [P113]\\
    \textit{``\textbf{Outlining} should help you structure your document before you begin.  \textbf{Writing} should check for spelling and grammar.  \textbf{Consulting} should make sure information is accurate.''} [P158]\\
    \textit{``The assistant could provide different services at different stages of the doc, such as during \textbf{editing} would provide with content suggestions; while \textbf{reviewing} it could provide with hints to include the right audience; on \textbf{publishing} it could help with Permission settings and privacy/compliance reviews; etc ...''} [P50]
\end{myquote}

%The common theme among this group of participants was that (1) writers do go through multiple phases during the writing process and (2) different phases involve different activities and hence require different skills and type of support.
\begin{comment}
\begin{myquote}{0.2in}
    \textit{``Designing a structure of a document and inviting/assigning contributors is different than editing/revising drafts.''} [P24]\\\\
    \textit{``the feedback required is different at each stage.''} [P118]
\end{myquote}
\end{comment}

A second round of qualitative coding of these responses resulted in identifying different activities that are associated with different phases of writing as perceived by our participants:
\begin{itemize}
    \item \emph{\textbf{Planning/Brainstorming Phase:}} Outlining/Diagramming [P36], section naming and setup [P46], help with structuring the document [P158]
    \item \emph{\textbf{Drafting Phase:}} Getting content or wording help [P44], structuring support to offload the mind [P63], support for sharing [P167]
    \item \emph{\textbf{Reviewing / Consulting Phase:}} notifications for formatting, grammar and spelling errors [P40], look of the document [P12], proofing [P75, P224], repetitive language usage [P167], highlighting unaddressed comments [P37], hints to include the right audience [P50, P133, P167], reminders to share or tag people [P224], fact checking [P123, P158], adding required references and sources [P133]
    \item \emph{\textbf{Finalizing / Publishing Phase:}} checking for broken paragraphs or tables before printing [P42], help with permission settings [P50], help with requesting required privacy and compliance reviews
\end{itemize}

In summary, writers recognize multiple phases during the writing process, they use a wide range of terminology to refer to them which can be grouped and mapped (at a high level) to the taxonomy of writing activities by Lowry et al \cite{lowry2004}. Similar to the previous theme of early versus late stages of document's evolution, different phases of writing are affiliated with different activities and the type of support should be tailored to the current phase of writing.
Finally, while these phases of writing can be seen as individual authors' mental state and hence are more complex to detect than early versus later stages of document evolution (as discussed in the previous subsection), we can see an overarching time-based ordering to these phases starting from brainstorming and outlining, moving to drafting, reviewing and finalizing.

%Please note that while there is no clear separation between these phases (e.g. end of outlining and early drafting, late drafting versus reviewing, etc), our participants do associate some phases to earlier stages of document evolution and other phases to the later stages.

\subsection{Modes of Writing}
Writing documents usually spans over multiple sessions of activity that are distributed over the lifetime of that document. 
When a writer attends to a document (representing the workspace), to do a particular task, they bring with them a general understanding of the current stage of a document (more clearly visible in SAW scenarios) and a basic idea of what to look for or what activity to do (see also Gutwin and Greenberg's \cite{gutwin2002} descriptive framework of workspace awareness for real-time groupware).

%A relevant theme to ``phases of writing'' is the intent of the writer who comes to a document at different stages during its lifetime.

%Similar to what Gutwin and Greenberg \cite{gutwin2002} describe in their descriptive framework of workspace awareness for real-time groupware, when a writer attends to a document (representing the workspace), to do a particular task, they bring with them a general understanding of the current stage of a document (more clearly visible in SAW scenarios) and a basic idea of what to look for or what activity to do.

%A common theme across a group of our participants was their intent or goal of attending to a document. They 
Our participants referred to different goals they have when they attend to a document at different times, and that based on this goal they are seeking different types of support from the system.

\begin{myquote}{0.2in}
    \textit{``Sometimes I'm just scanning a document for minor edits and other times I'm going full bore and ignoring small mistakes.''} [P15]\\
    \textit{``[when] writing [I'm] less focused on actual facts, where as reviewing will need to be very factual.''} [P123]\\
    \textit{``Sometimes you just need to get thoughts onto "paper" and other times you need to review feedback, clean up the content and get ready to publish.''} [P147]
\end{myquote}

%We note that the awareness of the writer's intent at the time they are attending to the document is already reflected in the writer's mental state in single author scenarios and the system can support this state by providing support that matches the intended activity.
A system can provide support that matches the intended activity: For example, hiding comments and change tracking annotations when the user is not in ``review mode'' or disabling editing when the user is in ``reading mode'' can help simplify the user's interaction with the writing environment and minimize changes by accident.

However, once we move to multi-author scenarios there is a need for a shared awareness of the document as the workspace, and the intent of a collaborator is impacted by this awareness.

\begin{myquote}{0.2in}
    \textit{``An ideal collaborative writing environment would allow users the choice of whether collaborators can view only or make edits to a document because the document should not be editable in certain situations.''} [P206]
\end{myquote}

%The final theme that was derived from our qualitative analysis is regarding the awareness of the stage that the shared document currently is and is predominantly visible in Collaborative Writing scenarios. The next subsection elaborates on this theme.

\subsection{Awareness of Document's Stage}
So far the three themes discussed above highlighted the importance of the detection of the current stage of a document or its corresponding writing phases to be able to provide writing support that is tailored to this stage. A distinct and interesting theme that was discovered through the qualitative coding of our survey responses was that the awareness of the stage of document's evolution is not only crucial for the system, i.e. an intelligent writing assistant, but is also crucial for collaborating authors who join a shared document at different stages of its lifetime. 

To clarify, while in single author scenarios a writer who attends to a document at some point in time generally has a good understanding of the current stage of a document and what the next steps should be, in collaborative writing scenarios developing and maintaining the workspace awareness is challenging \cite{gutwin2002}.

%In unpacking some of our participants responses we noticed a desire for a shared awareness of the document when multiple authors are involved. 

\begin{myquote}{0.2in}
    \textit{`` ...  At the end I need to know who all has access, if any feedback has been left, what stage the doc is in (in review, in implementation, locked, stale, etc.).''} [P81]\\
    \textit{``The requirements from collaboration will vary over the lifespan of the document from creation to delivery to retirement.''} [P80]
\end{myquote}

Gutwin and Greenberg \cite{gutwin2002} motivate the importance of workplace awareness for collaborative scenarios which can reduce effort, increase efficiency and reduce errors for the activities of collaboration.
%For example, awareness of the stage of document helps with coordination of and suggesting the ways new collaborators can contribute and assist the writing process.
Assisting others with their local tasks is an integral part of collaboration and one that also benefits from workspace awareness. Awareness in this situation is useful because it helps people determine what assistance is \textit{required} and what is \textit{appropriate}. This was confirmed by our participants:

%Our participants articulated that awareness of what stage the document is currently in can greatly help with anticipating what assistance is expected and appreciated by other collaborators.

\begin{myquote}{0.2in}
    \textit{``From the previous experiences, we tend to give more feedback in the beginning than the later when the content is mostly completed.''} [P195]
\end{myquote}

Some of our participants were proactive in suggesting ways that an intelligent system can detect the current stage of a document and share that information with other collaborators who attend the document at different times.

\begin{myquote}{0.2in}
    \textit{``[The system can track] the number of people with the document opened for edit.  Tracking the "shares" of the document to know when it's sent for review or edit. the intelligent assistant that provided me the prompts to share it for review or editing would know [the stage of the document] from the selections I make.''} [P172]
\end{myquote}

\subsection{Summary of Findings}
Our survey data provided different insights regarding how writers perceive the stages of a document evolution and what types of writing assistance is expected at these stages of document authoring.

The qualitative analysis of survey responses indicated that the writers in our population perceive a document stage in three different yet related ways: (1) temporal stages of document evolution; (2) phases of writing and (3) modes of writing. 

Given the complexity of the writing process and how different cognitive sub-processes of planning, translating and reviewing interact, we are yet to explore automatic methods that can detect these writing phases \cite{baaijen2012, leijten2013, conijn2019}.
However, our qualitative findings highlight an overarching temporal ordering of these writing phases and modes of writing as reflected in the mental model of our participants.
%that could be used as a first step towards characterizing stages of document authoring.

Further, our qualitative findings indicate that awareness of a current document's stage of evolution has implications for both users and the system.
While intelligent writing assistants can use this information to provide writing assistance to writers that is tailored to the current stage of the document, in collaborative scenarios, new collaborators who join a shared document at different points throughout the document's lifetime can better coordinate their next actions such that in can assist others by contributing to the current stage of writing. 

In the next section we revisit the notion of temporal stages of document evolution through a different lens, by characterizing differences in the users' interaction logs of a commercial writing application. Our main goal with this quantitative analysis is to verify our qualitative findings at scale and through a record of actual users interactions as they are writing documents.


==> sec.QualitativeAnalysis_short.tex <==
\section{Stage-aware Writing Assistance} 
\el{One thing that I note about this section and the next section is that the presentation of the methods/results are a bit different than is typical in most papers that present research studies. Usually, we write a methods section (or subsection here) followed by a results subsection. This allows the user (the reader) to separate in their mind what was done versus what was found.  I'm worried, here, that without this separation, it becomes hard to replicate the studies or to mentally track the switch between method vs results, which could negatively impact reviews.}

Our main research question is to investigate whether providing writing assistance that is tailored to the current stage of a document development is beneficial to the writers of that document.
To this end we need to better characterize two different aspects of \textit{stage-aware writing assistance}: 
\begin{enumerate}
    \item \textbf{Characterizing the stage of a document:} How are the stages of document evolution perceived by the writers?
    \item \textbf{Characterizing stage-appropriate writing assistance:} \\What writing assistance is beneficial at different stages of document evolution?
\end{enumerate}

% There are many open questions in this space including how common writing documents at the workplace is, what support is needed, what are the expectations of an intelligent writing tool and whether there is a need for tailored support at different stages of writing?

To address these two questions, we conducted a survey at a large technology company with a range of close-ended as well as open-ended questions. 
% Most research on the writing process has been carried out in the context of education. Thus, little focus has been put on the particularities which arise when the writing process is carried out by information workers who need to write documents as a part of their daily routine at the workplace.
The survey data helped us understand how enterprise workers approach the writing of a document, how the stages of document authoring are perceived by them and their expectations for types of writing assistance at these stages.

\subsection{Survey}
We distributed a survey within a large technology company and collected 175 responses (completion rate: 70\%).\bs{get response rate} %\rw{define this: it's not the same as response rate, correct? the way it's written suggests it's response rate, which was much lower than 70\%}. 
Our survey started with a section on demographics including job roles, number of current projects, team size, etc. The next section involved different questions regarding writing documents at the workplace which helped us verify whether writing documents at the workplace is a common practice, what tools are frequently used for writing documents and how often these documents involve other collaborators as well.

Respondents came from a diverse set of roles ranging from product managers and software developers to sales people and administrative assistants. Most respondents have worked at this company for over 5 years (63\%).  Multi-tasking on different projects was a common trend among them, with 75\% working on at least 3 projects.
\subsection{General Findings}
%Our survey data confirmed that writing documents is very common at the workplace. 
87\% of our respondents mentioned writing documents as a part of their work routine. They use a wide range of writing tools including Microsoft Word's Desktop client (89\%) and Online (Web-based) client (49\%), followed by Notepad / Notepad++ (19.3\%), OneNote (16\%), Overleaf / Sharelatex (11.1\%), Google Docs (8.2\%), etc.

Collaboration on these documents was also a common theme among our participants, with the majority (74\%) collaborating on at least 25\% of their documents.
Despite the commonality of collaborative writing, a closer examination of the qualitative responses (discussed below) indicated that the need for tailored support in different stages of document authoring is associated with both Single Author Writing (SAW) and Collaborative Writing (CW) scenarios. 
%While some of the participants talked about multi-author scenarios, the majority of responses could be applied to either of these scenarios. 
% Single author Writing (SAW) is defined as writing conducted by one individual that involves planning, drafting and reviewing (Lowry et al., 2004) Collaborative Writing (CW) builds on single-author writing by involving multiple people, thus increasing the complexity of the writing process (Galegher and Kraut, 1994).
\begin{myquote}{0.1in}
\textit{``in and ideal scenario I would just do some sort of content dump to the system and the system structures this text. So that I don't have to think about paragraphs, sections, where to put what etc. And then in later stages I want help with how to nicely formulate things. That's not only in a collaborative setting though.''} [P10]
\end{myquote}
As a first step towards understanding whether there is a need for different types of support at different stages of document evolution, in the next segment of our survey 
%included a series of questions to gauge real users perceptions and attitudes towards this concept. More formally, 
the participants were asked \textit{``Should an intelligent writing assistant provide different types of support at different stages of writing in the document?''} with a binary Yes / No response type.

Over 70\% of our participants expressed a need for different types of support at different stages of writing. The follow up open-ended questions to elaborate on their rationales for their response to this initial question revealed how these stages are perceived by the participants and that what support is needed at these stages. 

The responses to these questions were all analyzed using affinity diagramming. Data was initially clustered using open coding producing
19 clusters. Clusters were then analyzed using axial coding to identify overall themes in the data. We found that saturation for our
qualitative data occurred approximately after 80 participants, no
new clusters of information were identified. However, we continued
to cluster these responses for the remaining participants, particularly
attuned to data that might expand our clusters or add nuance to
our analysis. These clusters resulted in four broad themes, corresponding to different notions of the stage of a document as perceived by our participants and the utility of different types of writing assistance based on these stages.

The following three subsections elaborate on three different perceptions of a document's stage and the final subsection describes a different implication \rw{a different implication??} of awareness of the stage of a document that is essential for more effective collaboration over writing documents.

% (1) Supporting Early versus Later Stages of Document Evolution; (2) Supporting different phases of writing; (3) Supporting different modes or intents of writing; and (4) Awareness of Stage of Document is essential both for the intelligent System and the collaborating writers. We describe more details about these themes in the following subsections.

% better characterization of the

\begin{comment}
\subsection{Stage-based Support for both SAW and CW}
%Writers require different support at different stages of writing both in SAW and CW scenarios.

Single author Writing (SAW) is defined as writing conducted by one individual that involves planning, drafting and reviewing (Lowry et al., 2004)
Collaborative Writing (CW) involves multiple people, thus increasing the complexity of the writing process (Galegher and Kraut, 1994).

%While the complexity of CW scenarios is generally more amplified relative to SAW scenarios, 
A qualitative analysis of these survey responses indicated that the need for tailored support at different stages of writing is not only desirable for CW settings: the majority of responses are applicable to either of these scenarios. 
\begin{quote}
\textit{``in and ideal scenario I would just do some sort of content dump to the system and the system structures this text. So that I don't have to think about paragraphs, sections, where to put what etc. And then in later stages I want help with how to nicely formulate things. That's not only in a collaborative setting though.''} [P10]
\end{quote}

In unpacking the quote above we also see a time-based notion of stages of document writing that is further discussed in the following subsection.
\end{comment}

\subsection{Temporal Stages of Document Authoring}
The Stages Model of Writing \cite{rohman1965} focuses on the evolution of the text as an external by-product of the writing where the main three stages of pre-writing, writing, and rewriting are separated in time. 
% While more recent models (e.g. Flower and Hayes's model \cite{flower1984}) argue that a more realistic model of writing needs to focus on the mental processes involved in the writing process and that these mental processes are interleaved, hierarchically embedded and are not executed in a linear order, these models are indeed complementary and are not in conflict (Mitchell, 1996). 

%In fact, once we shift our view to the document as the by product of this process we can see some time based ordering of these high level stages of document evolution. 

This time-based ordering of document stages was shared amongst many of our participants who referred to them as early versus later stages of document writing. The qualitative analysis of their description of these early and late stages resulted in a novel characterization of these temporal stages and the writing phases and activities that are associated with each stage.
This characterization is based on observing notable differences in authors' perception of stages of document evolution and how it maps to temporal stages of document lifetime.
\bs{Ryen - I added this as a placeholder for clarifying what the novelty of this characterization is.}

%\rw{where is this characterization presented in the paper? is it what's next? if so, let's say that and how is it novel w.r.t. previous work?}
% The qualitative analysis of their description of these early and late stages resulted in a novel characterization of these temporal stages, which high level writing phases and low level writing activities are associated with them, and which types of writing assistance are appreciated in each stage and what support is perceived as interruption.

The early stages of writing are perceived to be highly focused and many participants expressed a desire for fewer interruptions and fewer system suggestions and notifications during these stages, particularly about minor fixes and improvements. 

%\advance\leftmargini 0.05em
\begin{myquote}{0.2in}
\textit{``I want fewer interruptions when i am focusing on adding content early in the document writing process.''} [P11]\\
\textit{``As someone who primarily writes documents in LaTeX, I like the ability to focus on writing the content without having to worry about formatting. Then only once the content is put down do I go back and tweak the look of the document. This allows me to focus on different aspects of the documents at different stages.''} [P12]
\end{myquote}

Later stages, on the other hand, are described as the time when most of the content has been added to the document and the writers can now focus on improving different aspects of the document during Reviewing, Copy-Editing and Finalizing phases.

\begin{myquote}{0.2in}
    \textit{``Document creation and document perfection are fundamentally different.  In my opinion, the best way to create a collaborative document is to get a rough draft made as quickly and dirtily as possible and then begin to improve it; different forms of assistance are required for each scenario.''} [P237]
\end{myquote}

Another interesting quality of later stages is that the document is known to be more ``mature'' with most of the content already included and structured. This quality has at least two different implications for what support can and should be provided at earlier versus later stages of writing. First, since in later stages the structure and the content of the document is highly stable the system can provide more end to end and global feedback as opposed to suggestions that are relevant to a specific part of the text only (e.g. identifying missing topics to be included versus spelling errors to be fixed). Second, with more content in place and a longer history of edits, intelligent writing assistants can be more reliable in predicting what support is needed.  
\begin{myquote}{0.2in}
    \textit{``When I'm actively working on creating the document I want suggestions around better writing style, but focused on what I'm doing at that moment.  Once the document is more mature I'd want feedback on the end to end document, not a specific word here or there.''} [P106]\\
    %\textit{``During the draft phase, there will be a lot of changes that just won't stick. At reviewing phase it would be helpful to objectively view the whole document to suggest improvements.''} [P207]\\
    %\textit{``Once a lot of content is in a document, a `bot' may be able to warn that you are going to change something that was just edited.''} [P77]\\\\
    \textit{``Intelligence should improve as the document matures.  The intent of the document, the subject matter, and the style of the document will become more clear as it evolves.''} [P78]
\end{myquote}

A different aspect of characterizing early and late stages of document evolution involved the high level phases of writing as well as low level activities that were associated with these stages.
The qualitative analysis of participants responses indicated that they associate different phases of writing including Planning, Outlining and Early Drafting to \textit{Early Stages of Writing}, whereas \textit{Later Stages} resonated with Reviewing and Copy-editing phases of writing. 

%As well, participants discussed a variety of activities in earlier stages of writing which revealed the types of support that are the most appreciated in these early stages. Among them, outlining and deciding on the structure of the document as well as searching for relevant content were perceived as early stage activities. 

Each of these phases of writing involves groups of activities that are similarly associated with earlier or later stages of document authoring. Among them, outlining and deciding on the structure of the document as well as searching for relevant content were perceived as early stage activities. Later stage activities, on the other hand, were focused on Reviewing including improving the document content (e.g., proofing and formatting), task management (e.g. addressing pending comments or TODO items) and collaboration (e.g. adding or communicating with collaborators through comments and change tracking functionalities), as well as Finalizing including fact checking, adding references, setting required permissions, etc. 

\begin{myquote}{0.2in}
    \textit{``When \textbf{getting started}, Outline or Structure help is needed \textbf{Later on} in the process, Editing, fact checking, adding references type of help is needed.''} [P84]\\
    \textit{``The needs at different stages may be very different. E.g. for structural changes, they better take place as \textbf{early} as possible; while for minor fixes or suggestions, they can come \textbf{later} when the body of text is by and large stable.''} [P64]
\end{myquote}

\begin{comment}
\begin{myquote}{0.2in}
    \textit{``Brainstorming and scope defining support \textbf{early on} that helps develop a basic outline and framework. It would be great for a writing assistant to help with the `starting from nothing' phase.''} [P98]\\
    \textit{``The needs at different stages may be very different. E.g. for structural changes, they better take place as \textbf{early} as possible; while for minor fixes or suggestions, they can come \textbf{later} when the body of text is by and large stable.''} [P64]\\
    \textit{``At the drafting stage, making sure the document is structured properly and all the bases are covered is paramount. At \textbf{later stages}, getting feedback and sign-off become much more important. It'd be great to more easily track changes.''} [P154]
    %\textit{``When \textbf{getting started}, Outline or Structure help is needed; \textbf{Later on} in the process, Editing, fact checking, adding references type of help is needed.''} [P84]\\\\
    %\textit{``\textbf{Early:} Focus and scope - needed at the beginning to understand what to write about and how much; this is often org dependent and the ability to create org-specific templates and help advice would be amazing.  \textbf{Mid:} Content analysis and comparison, to highlight style and completeness differences in different areas.  \textbf{Late:} Advice on structural features and cleanups that can save time and improve accessibility.''} [P219]\\\\
    %\textit{``Would be great to enter some notes and have an outline constructed. \textbf{Later} it would be great to have research done for me if I need a supporting quote or need a chart from another document. \textbf{Finally} it would help to have suggestions for alternatives to overused words.''} [P57]
\end{myquote}
\end{comment}

Finally, while supporting the activities that are associated to a certain stage is appreciated by the users, untimely system support can be perceived as \textit{distracting}, \textit{annoying}, or \textit{unnecessary}.
In particular, minor fixes, proofing and grammar fixes, collaborative activities such as commenting and change tracking are perceived as unhelpful nor appreciated during early stages of document evolution.
\begin{myquote}{0.2in}
    \textit{``Different actions and needs are required for each stage of writing; there is no need to suggest spacing and layout changes when I've just started writing down my thoughts (the text is "under-construction" and liable to change quickly).''} [P70]\\
    \textit{``Worrying about complete sentences and grammar while brainstorming would slow things down considerably ... but necessary for a final release.''} [P227]\\
    \textit{``Notifying me of grammar and spelling errors when I'm trying to get my thoughts out is really just a distraction. I prefer when these suggestions are made at a later editing stage.''} [P40]\\
    \textit{``Initial document writing is mainly non-collaborative, whereas later it's a matter of tweaking and improving with the feedback of others.''} [P178]
\end{myquote}


% Given that the main focus of later stages is on improving the document, different later stage activities are identified as Proofreading e.g. proofing and formatting, Task Management (e.g. addressing pending comments or TODO items), Collaborative Activities such as adding collaborators, communicating with collaborators through comments and change tracking functionalities, etc. as well as Reviewing and Finalizing activities including fact checking, adding references, setting required permissions, etc.

\begin{comment}
\begin{myquote}{0.2in}
    %\textit{``When getting started, Outline or Structure help is needed Later on in the process, Editing, fact checking, adding references type of help is needed ''} [P84]\\
    %\textit{``[In later stages] 1. Update me of unaddressed/unread comments that I should follow up on. 2. Help me identify similar comment available in other documents that I can use for reference.''} [P37]\\\\
    \textit{``At the drafting stage, making sure the document is structured properly and all the bases are covered is paramount. At later stages, getting feedback and sign-off become much more important. It'd be great to more easily track changes.''} [P154]\\
    \textit{``At the end of the writing process it is helpful to have a spelling and grammar check, with perhaps some suggestions on structure, yet I find suggestion DURING writing to be distracting.''} [P182]
   % \textit{``At the beginning providing table contents, title formats, and captioning. Later can add references, etc.''} [P194]\\
\end{myquote}
\end{comment}

%The main takeaways from what was discussed can be summarized as three implications for design:
The following three design implications are our main takeaway from the preceding analysis:
\begin{enumerate}
    \item Intelligent support should be provided based on the activities associated with the current stage of document evolution (i.e. early versus later stages).% in order to be appreciated by the writers.
    \item Authors are in a focused mode during earlier stage of writing and system interruptions should be minimized. 
    \item Authors can benefit from a higher level of control over the writing process in earlier stages with outlining, structuring, or searching functionalities that are provided on demand. During later stages intelligent systems can be more proactive in providing feedback and suggestions to improve the overall document quality.
\end{enumerate}

\subsection{Phases of Writing}
% According to Lowry et al's Taxonomy of Writing Activities \cite{lowry2004}, 
Different models of writing process \cite{flower1984, lowry2004} state that writers go through different phases throughout the document authoring process. These phases are characterized as brainstorming, outlining, drafting, reviewing, revising and copy editing \cite{lowry2004} or more broadly as planning, translating, and reviewing \cite{flower1984}. 
%This view of writing activities is largely inline with Flower and Hayes model that specifies planning, translating and reviewing as three main processes involved.

A qualitative analysis of our participants' responses reveals that the idea of going through different phases during the process of writing documents resonates with them and that they perceive the stage of the document based on these phases of writing. In fact these phases were described in a variety of terms:
\textit{``from document creation to document perfection''} [P237], \textit{``starting from nothing phase''} [P98], \textit{``Rough draft vs final draft''} [P?], \textit{``Draft, Editing, Polishing''} [P?, P220], \textit{``Creative or Brainstorming, `culling the first main draft', draft editing, reviewing, finalizing''} [P?] \textit{``Outlining, Writing, Consulting''} [P158], \textit{``Schedule (content requirements), Reminders \& goals, Refresh''} [P135], \textit{``early drafting, end of drafting, reviewing''} [P224] etc.

%Similar to the theme described in the previous subsection those participants who resonated with these phases of writing
% Participants described groups of activities that are associated with each phase and hence could use targeted support during that phase.
In probing the ways our participants described these phases of writing we noted an overarching temporal ordering to these phases as well as a variety of activities that are associated with each phase.

\begin{myquote}{0.2in}
    \textit{``%There are appropriate tasks for every phase that might not apply for all others and assistance in remembering them would be great. Like 
    Assistance for spellcheck/alignment  is much better suited to the end of \textbf{drafting}. Reminders to share or tag people are better suited for \textbf{reviewing}.''} [P224]\\
    \textit{``Different stages require different approaches: \textbf{drafting} is a ``throw in all ideas'', but \textbf{finalizing} is ``polish wording and structure''.  E.g.: Worrying about complete sentences and grammar while brainstorming would slow things down considerably … but necessary for a final release.''} [P227]\\
    %\textit{``\textbf{Brainstorming} vs. \textbf{Authoring} vs. \textbf{Finalizing} have very different needs.''} [P138]\\\\
   % \textit{``Writing stages differ: \textbf{Creative or brainstorming}. Culling the main \textbf{first draft}. \textbf{Draft editing} and \textbf{review}. \textbf{Finalization} of the document. Each involves a different skill set.''} [P113]\\
    \textit{``\textbf{Outlining} should help you structure your document before you begin.  \textbf{Writing} should check for spelling and grammar.  \textbf{Consulting} should make sure information is accurate.''} [P158]\\
    \textit{``The assistant could provide different services at \underline{different stages} \underline{of the doc}, such as during \textbf{editing} would provide with content suggestions; while \textbf{reviewing} it could provide with hints to include the right audience; on \textbf{publishing} it could help with Permission settings and privacy/compliance reviews''} [P50]
\end{myquote}

%The common theme among this group of participants was that (1) writers do go through multiple phases during the writing process and (2) different phases involve different activities and hence require different skills and type of support.
\begin{comment}
\begin{myquote}{0.2in}
    \textit{``Designing a structure of a document and inviting/assigning contributors is different than editing/revising drafts.''} [P24]\\\\
    \textit{``the feedback required is different at each stage.''} [P118]
\end{myquote}
\end{comment}

%\rw{is this the novel contribution flagged earlier in this section? if so, we need to better connect this to the earlier text}
A second round of qualitative coding of these responses resulted in identifying different activities that are associated with different phases of writing as perceived by our participants:
\begin{itemize}
    \item \emph{\textbf{Planning/Brainstorming Phase:}} Outlining/Diagramming [P36], section naming and setup [P46], help with structuring the document [P158]
    \item \emph{\textbf{Drafting Phase:}} Getting content or wording help [P44], structuring support to offload the mind [P63], support for sharing [P167]
    \item \emph{\textbf{Reviewing / Consulting Phase:}} notifications for formatting, grammar and spelling errors [P40], look of the document [P12], proofing [P75, P224], repetitive language usage [P167], highlighting unaddressed comments [P37], hints to include the right audience [P50, P133, P167], reminders to share or tag people [P224], fact checking [P123, P158], adding required references and sources [P133]
    \item \emph{\textbf{Finalizing / Publishing Phase:}} checking for broken paragraphs or tables before printing [P42], help with permission settings [P78], help with requesting required privacy and compliance reviews [P50]. %\rw{participant id?}
\end{itemize}

In summary, writers recognize multiple phases during the writing process, they use a wide range of terminology to refer to them which can be grouped and mapped (at a high level) to the taxonomy of writing activities by Lowry et al \cite{lowry2004}. Similar to the previous theme of early versus late stages of document's evolution, different phases of writing are affiliated with different activities and the type of support should be tailored to the current phase of writing.
Finally, while these phases of writing can be seen as individual authors' mental state and hence are more complex to detect than early versus later stages of document evolution (as discussed in the previous subsection), we can see an overarching time-based ordering to these phases starting from brainstorming and outlining, moving to drafting, reviewing and finalizing.

%Please note that while there is no clear separation between these phases (e.g. end of outlining and early drafting, late drafting versus reviewing, etc), our participants do associate some phases to earlier stages of document evolution and other phases to the later stages.

\subsection{Modes of Writing}
Writing documents usually spans over multiple sessions of activity that are distributed over the lifetime of that document. 
When a writer attends to a document (representing the workspace), to do a particular task, they bring with them a general understanding of the current stage of a document (more clearly visible in SAW scenarios) and a basic idea of what to look for or what activity to do (see also Gutwin and Greenberg's \cite{gutwin2002} descriptive framework of workspace awareness for real-time groupware).

%A relevant theme to ``phases of writing'' is the intent of the writer who comes to a document at different stages during its lifetime.

%Similar to what Gutwin and Greenberg \cite{gutwin2002} describe in their descriptive framework of workspace awareness for real-time groupware, when a writer attends to a document (representing the workspace), to do a particular task, they bring with them a general understanding of the current stage of a document (more clearly visible in SAW scenarios) and a basic idea of what to look for or what activity to do.

%A common theme across a group of our participants was their intent or goal of attending to a document. They 
Our participants referred to different goals they have when they attend to a document at different times, and that based on this goal they are seeking different types of support from the system.

\begin{myquote}{0.2in}
    \textit{``Sometimes I'm just scanning a document for minor edits and other times I'm going full bore and ignoring small mistakes.''} [P15]\\
    \textit{``[when] writing [I'm] less focused on actual facts, where as reviewing will need to be very factual.''} [P123]\\
    \textit{``Sometimes you just need to get thoughts onto "paper" and other times you need to review feedback, clean up the content and get ready to publish.''} [P147]
\end{myquote}

%We note that the awareness of the writer's intent at the time they are attending to the document is already reflected in the writer's mental state in single author scenarios and the system can support this state by providing support that matches the intended activity.
A system can provide support that matches the intended activity: For example, hiding comments and change tracking annotations when the user is not in ``review mode'' or disabling editing when the user is in ``reading mode'' can help simplify the user's interaction with the writing environment and minimize changes by accident.

However, once we move to multi-author scenarios there is a need for a shared awareness of the document as the workspace, and the intent of a collaborator is impacted by this awareness.

\begin{myquote}{0.2in}
    \textit{``An ideal collaborative writing environment would allow users the choice of whether collaborators can view only or make edits to a document because the document should not be editable in certain situations.''} [P206]
\end{myquote}

%The final theme that was derived from our qualitative analysis is regarding the awareness of the stage that the shared document currently is and is predominantly visible in Collaborative Writing scenarios. The next subsection elaborates on this theme.

\subsection{Awareness of Document's Stage}
So far, the three themes discussed above highlighted the importance of the detection of the current stage of a document or its corresponding writing phases to be able to provide writing support that is tailored to this stage. A distinct and interesting theme that was discovered through the qualitative coding of our survey responses was that the awareness of the stage of document's evolution is not only crucial for the system, i.e., an intelligent writing assistant, but is also crucial for collaborating authors who join a shared document at different stages of its lifetime. 

To clarify, while in single author scenarios a writer who attends to a document at some point in time generally has a good understanding of the current stage of a document and what the next steps should be, in collaborative writing scenarios developing and maintaining the workspace awareness is challenging \cite{gutwin2002}.

%In unpacking some of our participants responses we noticed a desire for a shared awareness of the document when multiple authors are involved. 

\begin{myquote}{0.2in}
    \textit{``At the end I need to know who all has access, if any feedback has been left, \underline{what stage the doc is in} (in review, in implementation, locked, stale, etc.).''} [P81]\\
    \textit{``The requirements from collaboration will vary over the lifespan of the document from creation to delivery to retirement.''} [P80]
\end{myquote}
Gutwin and Greenberg \cite{gutwin2002} motivate the importance of workplace awareness for collaborative scenarios which can reduce effort, increase efficiency, and reduce errors for the activities of collaboration.
%For example, awareness of the stage of document helps with coordination of and suggesting the ways new collaborators can contribute and assist the writing process.
Assisting others with their local tasks is an integral part of collaboration and one that also benefits from workspace awareness. Awareness in this situation is useful because it helps people determine what assistance is \textit{required} and what is \textit{appropriate}. This was confirmed by our participants:

%Our participants articulated that awareness of what stage the document is currently in can greatly help with anticipating what assistance is expected and appreciated by other collaborators.

\begin{myquote}{0.2in}
    \textit{``From the previous experiences, we tend to give more feedback in the beginning than the later when the content is mostly completed.''} [P195]
\end{myquote}

Some of our participants were proactive in suggesting ways that an intelligent system can detect the current stage of a document and share that information with other collaborators who attend the document at different times.

\begin{myquote}{0.2in}
    \textit{``[The system can track] the number of people with the document opened for edit.  Tracking the "shares" of the document to know when it's sent for review or edit. the intelligent assistant that provided me the prompts to share it for review or editing would know [the stage of the document] from the selections I make.''} [P172]
\end{myquote}

\subsection{Summary of Findings}
Our survey data provided a range of insights regarding how writers perceive the stages of a document evolution and what types of writing assistance is expected at these stages of document authoring.

The qualitative analysis of survey responses indicated that the writers in our population perceive a document stage in three different, yet related ways: (1) temporal stages of document evolution; (2) phases of writing, and (3) modes of writing. 

Given the complexity of the writing process and how different cognitive sub-processes of planning, translating and reviewing interact, we are yet to explore automatic methods that can detect these writing phases \cite{baaijen2012, leijten2013, conijn2019}.
However, our qualitative findings highlight an overarching temporal ordering of these writing phases and modes of writing as reflected in the mental model of our participants.
%that could be used as a first step towards characterizing stages of document authoring.
Further, our qualitative findings indicate that awareness of a current document's stage of evolution has implications for both \textcolor{red}{authors} 
%\rw{we should be consistent in how we refer to people in the study - i prefer authors, but i've also seen users and writers used in the paper} 
and the system.
While intelligent writing assistants can use this information to provide writing assistance to writers that is tailored to the current stage of the document, in collaborative scenarios, new collaborators who join a shared document at different points throughout the document's lifetime can better coordinate their next actions such that in can assist others by contributing to the current stage of writing. 

In the next section, we revisit the notion of temporal stages of document evolution through a different lens, by characterizing differences in user interaction logs of a commercial writing application. Our main goal with this quantitative analysis is to verify our qualitative findings at Web-scale and through a record of actual users' interactions as they are writing documents.


==> sec.QualitativeFindings.tex <==
\section{Qualitative Findings} 
\label{sec:qualfind}
%As a first step towards characterizing stages of document authoring as well as how stage-based writing assistance is perceived by authors we analyzed the data captured by our survey.

We analyzed our survey response data with the goal of characterizing stages of document authoring as well as learning how stage-based writing assistance is perceived by authors

We found that 87\% of respondents mentioned writing documents as a part of their work routine. They use a wide range of writing tools including Microsoft Word's Desktop client (89\%) and Online (Web-based) client (49\%),  Notepad / Notepad++ (19.3\%), OneNote (16\%), Overleaf / Sharelatex (11.1\%), Google Docs (8.2\%), and others.

Collaboration on these documents was a common theme, with the majority of participants (74\%) collaborating on at least 25\% of their documents.
%Despite the popularity of collaborative writing, 
A closer examination of the qualitative responses (discussed below) indicated that the need for tailored support in different stages of document authoring is associated with both Single Author Writing (SAW) and Collaborative Writing (CW) scenarios. 
%While some of the participants talked about multi-author scenarios, the majority of responses could be applied to either of these scenarios. 
% Single author Writing (SAW) is defined as writing conducted by one individual that involves planning, drafting and reviewing (Lowry et al., 2004) Collaborative Writing (CW) builds on single-author writing by involving multiple people, thus increasing the complexity of the writing process (Galegher and Kraut, 1994).
\begin{myquote}{0.1in}
\textit{``in an ideal scenario I would just do some sort of content dump to the system and the system structures this text. So that I don't have to think about paragraphs, sections, where to put what etc. And then in later stages I want help with how to nicely formulate things. That's not only in a collaborative setting though.''} [P10]
\end{myquote}
%As a first step towards understanding 
To understand whether there is a need for different types of support at different stages of document evolution, 
%in the next segment of our survey 
%included a series of questions to gauge real users perceptions and attitudes towards this concept. More formally, 
the participants were asked \textit{``Should an intelligent writing assistant provide different types of support at different stages of writing in the document?''} with a binary Yes / No response type.

Over 70\% of participants expressed a need for different types of support at different stages of writing. 
%The follow up open-ended questions 
%to elaborate on their rationales for their response to this initial question 
%revealed how these stages are perceived by the participants and what support is needed at these stages. 

% The responses to these questions were all analyzed using affinity diagramming. Data was initially clustered using open coding producing 19 clusters. Clusters were then analyzed using axial coding to identify overall themes in the data. We found that saturation for our qualitative data occurred approximately after 80 participants, no new clusters of information were identified. However, we continued to cluster these responses for the remaining participants, particularly attuned to data that might expand our clusters or add nuance to our analysis. 
The qualitative analysis of the follow up open-ended questions (as described in Section \ref{Survey}) resulted in four broad themes, corresponding to different notions of the stage of a document as perceived by our participants and the utility of different types of writing assistance based on these stages.

The following three subsections elaborate on different perceptions of a document's stage and their corresponding writing activities, which has implications for designing stage-aware writing assistants. The final subsection provides a different perspective on the utility of document stage awareness, which is essential for more effective collaborative writing scenarios.

% (1) Supporting Early versus Later Stages of Document Evolution; (2) Supporting different phases of writing; (3) Supporting different modes or intents of writing; and (4) Awareness of Stage of Document is essential both for the intelligent System and the collaborating writers. We describe more details about these themes in the following subsections.

% better characterization of the

\begin{comment}
\subsection{Stage-based Support for both SAW and CW}
%Writers require different support at different stages of writing both in SAW and CW scenarios.

Single author Writing (SAW) is defined as writing conducted by one individual that involves planning, drafting and reviewing (Lowry et al., 2004)
Collaborative Writing (CW) involves multiple people, thus increasing the complexity of the writing process (Galegher and Kraut, 1994).

%While the complexity of CW scenarios is generally more amplified relative to SAW scenarios, 
A qualitative analysis of these survey responses indicated that the need for tailored support at different stages of writing is not only desirable for CW settings: the majority of responses are applicable to either of these scenarios. 
\begin{quote}
\textit{``in and ideal scenario I would just do some sort of content dump to the system and the system structures this text. So that I don't have to think about paragraphs, sections, where to put what etc. And then in later stages I want help with how to nicely formulate things. That's not only in a collaborative setting though.''} [P10]
\end{quote}

In unpacking the quote above we also see a time-based notion of stages of document writing that is further discussed in the following subsection.
\end{comment}

\subsection{Temporal Stages of Document Authoring}
The Stages Model of Writing \cite{rohman1965} focuses on the evolution of the text as an external by-product of the writing where the main three stages of pre-writing, writing, and rewriting are separated in time. 
% While more recent models (e.g. Flower and Hayes's model \cite{flower1984}) argue that a more realistic model of writing needs to focus on the mental processes involved in the writing process and that these mental processes are interleaved, hierarchically embedded and are not executed in a linear order, these models are indeed complementary and are not in conflict (Mitchell, 1996). 

%In fact, once we shift our view to the document as the by product of this process we can see some time based ordering of these high level stages of document evolution. 

This notion of document stages resonated with many of our participants, who referred to them as early versus later stages of document writing. 
Qualitative analysis of the respondent's descriptions of these temporal stages revealed how they are conceptualized and what writing phases and activities are associated with each stage.
%resulted in a novel characterization of these temporal stages and the writing phases and activities that are associated with each stage.
%This characterization is based on observing notable differences in authors' perception of stages of document evolution and how it maps to temporal stages of document lifetime.
%\bs{Ryen - I added this as a placeholder for clarifying what the novelty of this characterization is.}
%\mg{I just got rid of the novelty claim to save space...}
%\rw{where is this characterization presented in the paper? is it what's next? if so, let's say that and how is it novel w.r.t. previous work?}
% The qualitative analysis of their description of these early and late stages resulted in a novel characterization of these temporal stages, which high level writing phases and low level writing activities are associated with them, and which types of writing assistance are appreciated in each stage and what support is perceived as interruption.

The early stages of writing are perceived to be highly focused and many participants expressed a desire for fewer system suggestions and notifications during these stages, particularly about minor fixes and improvements. 

%\advance\leftmargini 0.05em
\begin{myquote}{0.2in}
\textit{``I want fewer interruptions when i am focusing on adding content early in the document writing process.''} [P11]\\
\textit{``As someone who primarily writes documents in LaTeX, I like the ability to focus on writing the content without having to worry about formatting. Then only once the content is put down do I go back and tweak the look of the document. This allows me to focus on different aspects of the documents at different stages.''} [P12]
\end{myquote}

Later stages, on the other hand, are described as the time when most of the content has been added to the document and the writers can now focus on improving different aspects of the document during Reviewing, Copy-Editing and Finalizing phases.

\begin{myquote}{0.2in}
    \textit{``Document creation and document perfection are fundamentally different.  In my opinion, the best way to create a collaborative document is to get a rough draft made as quickly and dirtily as possible and then begin to improve it; different forms of assistance are required for each scenario.''} [P237]
\end{myquote}

At later stages the document is more ``mature'' with most of the content already included and structured. This quality has at least two different implications for what support can and should be provided at earlier versus later stages of writing. First, in later stages 
%the structure and the content of the document is highly stable 
the system can provide more end to end and global feedback as opposed to local suggestions
%that are relevant to a specific part of the text only 
(e.g., identifying missing topics to be included versus spelling errors to be fixed). Second, with more content in place and a longer history of edits, intelligent writing assistants can be more reliable in predicting what support is needed.  
\begin{myquote}{0.2in}
    \textit{``When I'm actively working on creating the document I want suggestions around better writing style, but focused on what I'm doing at that moment.  Once the document is more mature I'd want feedback on the end to end document, not a specific word here or there.''} [P106]\\
    %\textit{``During the draft phase, there will be a lot of changes that just won't stick. At reviewing phase it would be helpful to objectively view the whole document to suggest improvements.''} [P207]\\
    %\textit{``Once a lot of content is in a document, a `bot' may be able to warn that you are going to change something that was just edited.''} [P77]\\\\
    \textit{``Intelligence should improve as the document matures.  The intent of the document, the subject matter, and the style of the document will become more clear as it evolves.''} [P78]
\end{myquote}

%A different aspect of characterizing early and late stages of document evolution involved the high level phases of writing as well as low level activities that were associated with these stages.
The qualitative analysis of participant responses indicated that they associate different phases of writing, including Planning, Outlining, and Early Drafting to \textit{Early Stages of Writing}, whereas \textit{Later Stages} resonated with Reviewing and Copy-editing phases.% of writing. 

%As well, participants discussed a variety of activities in earlier stages of writing which revealed the types of support that are the most appreciated in these early stages. Among them, outlining and deciding on the structure of the document as well as searching for relevant content were perceived as early stage activities. 

Each of these phases of writing involves specific groups of activities. 
%that are similarly associated with earlier or later stages of document authoring. 
Among them, outlining and deciding on the structure of the document as well as searching for relevant content were perceived as early stage activities. Later stage activities were focused on Reviewing including improving the document content (e.g., proofing and formatting), task management (e.g., addressing pending comments or TODO items) and collaboration (e.g., adding or communicating with collaborators through comments and change tracking functionalities), as well as Finalizing including fact checking, adding references, setting required permissions, etc. 

\begin{myquote}{0.2in}
    \textit{``When \textbf{getting started}, Outline or Structure help is needed \textbf{Later on} in the process, Editing, fact checking, adding references type of help is needed.''} [P84]\\
    \textit{``The needs at different stages may be very different. E.g. for structural changes, they better take place as \textbf{early} as possible; while for minor fixes or suggestions, they can come \textbf{later} when the body of text is by and large stable.''} [P64]
\end{myquote}

\begin{comment}
\begin{myquote}{0.2in}
    \textit{``Brainstorming and scope defining support \textbf{early on} that helps develop a basic outline and framework. It would be great for a writing assistant to help with the `starting from nothing' phase.''} [P98]\\
    \textit{``The needs at different stages may be very different. E.g. for structural changes, they better take place as \textbf{early} as possible; while for minor fixes or suggestions, they can come \textbf{later} when the body of text is by and large stable.''} [P64]\\
    \textit{``At the drafting stage, making sure the document is structured properly and all the bases are covered is paramount. At \textbf{later stages}, getting feedback and sign-off become much more important. It'd be great to more easily track changes.''} [P154]
    %\textit{``When \textbf{getting started}, Outline or Structure help is needed; \textbf{Later on} in the process, Editing, fact checking, adding references type of help is needed.''} [P84]\\\\
    %\textit{``\textbf{Early:} Focus and scope - needed at the beginning to understand what to write about and how much; this is often org dependent and the ability to create org-specific templates and help advice would be amazing.  \textbf{Mid:} Content analysis and comparison, to highlight style and completeness differences in different areas.  \textbf{Late:} Advice on structural features and cleanups that can save time and improve accessibility.''} [P219]\\\\
    %\textit{``Would be great to enter some notes and have an outline constructed. \textbf{Later} it would be great to have research done for me if I need a supporting quote or need a chart from another document. \textbf{Finally} it would help to have suggestions for alternatives to overused words.''} [P57]
\end{myquote}
\end{comment}

Finally, while supporting the activities that are associated with a certain stage was appreciated by survey respondents, untimely system support can be perceived as \textit{distracting}, \textit{annoying}, or \textit{unnecessary}.
In particular, minor fixes, proofing and grammar fixes, collaborative activities such as commenting and change tracking are perceived as unhelpful during early stages of document evolution.
\begin{myquote}{0.2in}
    \textit{``Different actions and needs are required for each stage of writing; there is no need to suggest spacing and layout changes when I've just started writing down my thoughts (the text is "under-construction" and liable to change quickly).''} [P70]\\
    \textit{``Worrying about complete sentences and grammar while brainstorming would slow things down considerably ... but necessary for a final release.''} [P227]\\
    \textit{``Notifying me of grammar and spelling errors when I'm trying to get my thoughts out is really just a distraction. I prefer when these suggestions are made at a later editing stage.''} [P40]\\
    \textit{``Initial document writing is mainly non-collaborative, whereas later it's a matter of tweaking and improving with the feedback of others.''} [P178]
\end{myquote}


% Given that the main focus of later stages is on improving the document, different later stage activities are identified as Proofreading e.g. proofing and formatting, Task Management (e.g. addressing pending comments or TODO items), Collaborative Activities such as adding collaborators, communicating with collaborators through comments and change tracking functionalities, etc. as well as Reviewing and Finalizing activities including fact checking, adding references, setting required permissions, etc.

\begin{comment}
\begin{myquote}{0.2in}
    %\textit{``When getting started, Outline or Structure help is needed Later on in the process, Editing, fact checking, adding references type of help is needed ''} [P84]\\
    %\textit{``[In later stages] 1. Update me of unaddressed/unread comments that I should follow up on. 2. Help me identify similar comment available in other documents that I can use for reference.''} [P37]\\\\
    \textit{``At the drafting stage, making sure the document is structured properly and all the bases are covered is paramount. At later stages, getting feedback and sign-off become much more important. It'd be great to more easily track changes.''} [P154]\\
    \textit{``At the end of the writing process it is helpful to have a spelling and grammar check, with perhaps some suggestions on structure, yet I find suggestion DURING writing to be distracting.''} [P182]
   % \textit{``At the beginning providing table contents, title formats, and captioning. Later can add references, etc.''} [P194]\\
\end{myquote}
\end{comment}

%The main takeaways from what was discussed can be summarized as three implications for design:
The following three design implications are our main takeaways from the preceding analysis:
\begin{enumerate}
    \item Intelligent support should be provided based on the activities associated with the current stage of document evolution (i.e., early versus later stages).% in order to be appreciated by the writers.
    \item Authors are in a focused mode during earlier stage of writing and system interruptions should be minimized. 
    \item Authors can benefit from a higher level of control over the writing process in earlier stages with outlining, structuring, or searching functionalities that are provided on demand. During later stages, intelligent systems can be more proactive in providing feedback and suggestions to improve the overall document quality.
\end{enumerate}
\vspace{-1mm}
\subsection{Phases of Writing}
% According to Lowry et al's Taxonomy of Writing Activities \cite{lowry2004}, 
Different models of the writing process \cite{flower1984, lowry2004} state that writers go through different phases throughout the document authoring process. These phases are characterized as brainstorming, outlining, drafting, reviewing, revising and copy editing \cite{lowry2004} or more broadly as planning, translating, and reviewing \cite{flower1984}. 
%This view of writing activities is largely inline with Flower and Hayes model that specifies planning, translating and reviewing as three main processes involved.

Our participants' responses reveal that the idea of going through different phases during the process of writing documents resonates with them and that they perceive the stage of the document based on these phases of writing. In fact these phases were described in a variety of terms:
\textit{``from document creation to document perfection''} [P237], \textit{``starting from nothing phase''} [P98], \textit{``Rough draft vs final draft''} [P79], \textit{``Draft, Editing, Polishing''} [P93, P220], \textit{``Creative or Brainstorming, `culling the first main draft', draft editing, reviewing, finalizing''} [P113] \textit{``Outlining, Writing, Consulting''} [P158], \textit{``Schedule (content requirements), Reminders \& goals, Refresh''} [P135], \textit{``early drafting, end of drafting, reviewing''} [P224], etc.

%Similar to the theme described in the previous subsection those participants who resonated with these phases of writing
% Participants described groups of activities that are associated with each phase and hence could use targeted support during that phase.
In probing the ways our participants described these phases of writing we noted an overarching temporal ordering to these phases as well as a variety of activities that are associated with each phase.

\begin{quote}
    \textit{``%There are appropriate tasks for every phase that might not apply for all others and assistance in remembering them would be great. Like 
    Assistance for spellcheck/alignment  is much better suited to the end of \textbf{drafting}. Reminders to share or tag people are better suited for \textbf{reviewing}.''} [P224]\\
    \textit{``Different stages require different approaches: \textbf{drafting} is a ``throw in all ideas'', but \textbf{finalizing} is ``polish wording and structure''.  E.g.: Worrying about complete sentences and grammar while brainstorming would slow things down considerably ... but necessary for a final release.''} [P227]\\
    %\textit{``\textbf{Brainstorming} vs. \textbf{Authoring} vs. \textbf{Finalizing} have very different needs.''} [P138]\\\\
   % \textit{``Writing stages differ: \textbf{Creative or brainstorming}. Culling the main \textbf{first draft}. \textbf{Draft editing} and \textbf{review}. \textbf{Finalization} of the document. Each involves a different skill set.''} [P113]\\
    \textit{``\textbf{Outlining} should help you structure your document before you begin.  \textbf{Writing} should check for spelling and grammar.  \textbf{Consulting} should make sure information is accurate.''} [P158]\\
    \textit{``The assistant could provide different services at \underline{different stages} \underline{of the doc}, such as during \textbf{editing} would provide with content suggestions; while \textbf{reviewing} it could provide with hints to include the right audience; on \textbf{publishing} it could help with Permission settings and privacy/compliance reviews''} [P50]
\end{quote}

%The common theme among this group of participants was that (1) writers do go through multiple phases during the writing process and (2) different phases involve different activities and hence require different skills and type of support.
\begin{comment}
\begin{myquote}{0.2in}
    \textit{``Designing a structure of a document and inviting/assigning contributors is different than editing/revising drafts.''} [P24]\\\\
    \textit{``the feedback required is different at each stage.''} [P118]
\end{myquote}
\end{comment}

%\rw{is this the novel contribution flagged earlier in this section? if so, we need to better connect this to the earlier text}
A second round of qualitative coding of these responses resulted in identifying different activities that are associated with different phases of writing as perceived by our participants:
\begin{itemize}
    \item \emph{\textbf{Planning/Brainstorming Phase:}} Outlining/Diagramming [P36], section naming and setup [P46], help with structuring the document [P158]
    \item \emph{\textbf{Drafting Phase:}} Getting content or wording help [P44], structuring support to offload the mind [P63], support for sharing [P167]
    \item \emph{\textbf{Reviewing / Consulting Phase:}} notifications for formatting, grammar and spelling errors [P40], look of the document [P12], proofing [P75, P224], repetitive language usage [P167], highlighting unaddressed comments [P37], hints to include the right audience [P50, P133, P167], reminders to share or tag people [P224], fact checking [P123, P158], adding required references and sources [P133]
    \item \emph{\textbf{Finalizing / Publishing Phase:}} checking for broken paragraphs or tables before printing [P42], help with permission settings [P78], help with requesting required privacy and compliance reviews [P50]. %\rw{participant id?}
\end{itemize}

In summary, writers recognize multiple phases during the writing process. They also use a wide range of terminology to refer to these phases, which can be grouped and mapped (at a high level) to the taxonomy of writing activities from \citet{lowry2004}. Similar to the previous theme of early versus late stages of document's evolution, different phases of writing are affiliated with different activities and the type of support should be tailored to the current phase of writing.
Finally, while these phases of writing can be seen as individual authors' mental states and hence are more complex to detect than early versus later stages of document evolution (as discussed in the previous subsection), we can see an overarching time-based ordering to these phases starting from brainstorming and outlining, moving to drafting, reviewing, and finalizing.
\vspace{-1mm}
%Please note that while there is no clear separation between these phases (e.g. end of outlining and early drafting, late drafting versus reviewing, etc), our participants do associate some phases to earlier stages of document evolution and other phases to the later stages.

\subsection{Modes of Writing}
Writing documents usually spans multiple sessions of activity that are distributed over document lifetimes. 
When a writer attends to a document (representing the workspace), to do a particular task, they bring with them a general understanding of the current stage of a document (more clearly visible in SAW scenarios) and a basic idea of what to look for or what activity to do (see also Gutwin and Greenberg's \cite{gutwin2002} descriptive framework of workspace awareness for real-time groupware).

%A relevant theme to ``phases of writing'' is the intent of the writer who comes to a document at different stages during its lifetime.

%Similar to what Gutwin and Greenberg \cite{gutwin2002} describe in their descriptive framework of workspace awareness for real-time groupware, when a writer attends to a document (representing the workspace), to do a particular task, they bring with them a general understanding of the current stage of a document (more clearly visible in SAW scenarios) and a basic idea of what to look for or what activity to do.

%A common theme across a group of our participants was their intent or goal of attending to a document. They 
Our participants referred to different goals they have when they attend to a document at different times, and that based on this goal they are seeking different types of support from the system.
\vspace{-0.5mm}
\begin{myquote}{0.2in}
    \textit{``Sometimes I'm just scanning a document for minor edits and other times I'm going full bore and ignoring small mistakes.''} [P15]\\
    \textit{``[when] writing [I'm] less focused on actual facts, where as reviewing will need to be very factual.''} [P123]\\
    \textit{``Sometimes you just need to get thoughts onto "paper" and other times you need to review feedback, clean up the content and get ready to publish.''} [P147]
\end{myquote}

%We note that the awareness of the writer's intent at the time they are attending to the document is already reflected in the writer's mental state in single author scenarios and the system can support this state by providing support that matches the intended activity.
A system can provide support that matches the intended activity: For example, hiding comments and change tracking annotations when the user is not in ``review mode'' or disabling editing when the user is in ``reading mode'' can help simplify the user's interaction with the writing environment and minimize accidental changes.

However, once we move to multi-author scenarios there is a need for a shared awareness of the document as the workspace, and the intent of a collaborator is impacted by this awareness.

\begin{myquote}{0.2in}
    \textit{``An ideal collaborative writing environment would allow users the choice of whether collaborators can view only or make edits to a document because the document should not be editable in certain situations.''} [P206]
\end{myquote}

%The final theme that was derived from our qualitative analysis is regarding the awareness of the stage that the shared document currently is and is predominantly visible in Collaborative Writing scenarios. The next subsection elaborates on this theme.

\subsection{Awareness of Document's Stage}
So far, the three themes discussed above highlighted the importance of the detection of the current stage of a document or its corresponding writing phases to be able to provide writing support that is tailored to this stage. A distinct and interesting theme that was discovered through the qualitative coding of our survey responses was that the awareness of the stage of document's evolution is not only crucial for the system, i.e., an intelligent writing assistant, but is also crucial for collaborating authors who join a shared document at different stages of its lifetime. 

Tools to communicate stage awareness are particularly needed during collaborative authoring. In single author scenarios an author who attends to a document at some point in time generally has a good understanding of the current stage of a document and what the next steps should be, whereas in collaborative writing scenarios developing and maintaining this workspace awareness is challenging \cite{gutwin2002}.

%In unpacking some of our participants responses we noticed a desire for a shared awareness of the document when multiple authors are involved. 

\begin{myquote}{0.18in}
    \textit{``At the end I need to know who all has access, if any feedback has been left, \underline{what stage the doc is in} (in review, in implementation, locked, stale, etc.).''} [P81]\\
    \textit{``The requirements from collaboration will vary over the lifespan of the document from creation to delivery to retirement.''} [P80]
\end{myquote}
\citet{gutwin2002} motivate the importance of workplace awareness for collaborative scenarios which can reduce effort, increase efficiency, and reduce errors for the activities of collaboration.
%For example, awareness of the stage of document helps with coordination of and suggesting the ways new collaborators can contribute and assist the writing process.
Assisting others with their local tasks is an integral part of collaboration and one that also benefits from workspace awareness. Awareness in this situation is useful because it helps people determine what assistance is \textit{required} and what is \textit{appropriate}. This was confirmed by our participants:

%Our participants articulated that awareness of what stage the document is currently in can greatly help with anticipating what assistance is expected and appreciated by other collaborators.

\begin{myquote}{0.18in}
    \textit{``From the previous experiences, we tend to give more feedback in the beginning than the later when the content is mostly completed.''} [P195]
\end{myquote}

Some of our participants were proactive in suggesting ways that an intelligent system can detect the current stage of a document and share that information with other collaborators who attend the document at different times:

\begin{myquote}{0.18in}
    \textit{``[The system can track] the number of people with the document opened for edit.  Tracking the "shares" of the document to know when it's sent for review or edit. the intelligent assistant that provided me the prompts to share it for review or editing would know [the stage of the document] from the selections I make.''} [P172]
\end{myquote}

\subsection{Summary of Findings}
Our survey data provided a range of insights regarding how authors perceive the stages of a document evolution and what types of writing assistance is expected at these stages of document authoring.

The qualitative analysis of survey responses indicated that the writers in our population perceive a document stage in three different, yet related ways: (1) temporal stages of document evolution; (2) phases of writing, and (3) modes of writing. 

Given the complexity of the writing process and how different cognitive sub-processes of planning, translating and reviewing interact, we are yet to explore automatic methods that can detect these writing phases \cite{baaijen2012, leijten2013, conijn2019}.
However, our qualitative findings highlight an overarching temporal ordering of these writing phases and modes of writing as reflected in the mental model of our participants.
%that could be used as a first step towards characterizing stages of document authoring.
Further, our qualitative findings indicate that awareness of a current document's stage of evolution has implications for both authors 
%\rw{we should be consistent in how we refer to people in the study - i prefer authors, but i've also seen users and writers used in the paper} 
and the system.
While intelligent writing assistants can use this information to provide writing assistance to writers that is tailored to the current stage of the document, in collaborative scenarios, new collaborators who join a shared document at different points throughout the document's lifetime can better coordinate their next actions such that it can assist others by contributing to the current stage of writing. 

In the next section, we revisit the notion of temporal stages of document evolution through a different lens, by characterizing differences in user interaction logs of a commercial writing application. Our main goal with this quantitative analysis is to verify our qualitative findings at Web-scale and through a record of actual users' interactions as they are writing documents.


==> sec.QuantitativeAnalysis.tex <==
\section{Stages of Document Evolution in User Logs}
%Our survey data highlighted different aspects of stages of documents writing as perceived by the information workers in our population and what support is needed at these stages.

%In this section we revisit our main research question of whether writers interactions with the writing environment is indeed different over different stages of document's evolution through a different lens, by characterizing differences in the users' interaction logs of a commercial writing application.

Our quantitative analysis seeks to answer two main research questions:\\
\rw{These questions should be formatted in the same way as those at start of Section 3}
1. Are there differences in the magnitude of user's interaction at different stages of the document evolution?\\
2. What types of writing activities are pertaining to earlier versus later stages of document evolution?

% \begin{verbatim}
% - TODO: Add a description of our logs.
% \end{verbatim}
\subsection{Data}
\label{Data}

\rw{Do these data come from the online client (WAC)? If so, we should certainly mention that as it strengthens the connection to the web}\bs{I believe the data is from the desktop client.}
In order to investigate these two research questions, we analyzed a sample of the anonymous interaction logs from users of a major commercial writing application \footnote{name suppressed for blind reviewing} over a three month period from February 1st to April 30th, 2019. 

To create this dataset, we collected a subset of document candidates in English from the US market that were created within a 2 week period from February 1st to 15th. For these documents we collected logs of user interactions with different functionalities available through the application UI \footnote{This modern, widely used word processing application provides standard functionalities including copy-paste, formatting, commenting, change tracking, etc.}.
Our sample consists of about 16 million document candidates and about 16.6 million users who accessed these documents.
%\bs{Elaborating on Consumers versus Contributors?}

Our interaction logs contain neither any textual data, nor any information about the users besides a system generated ID that can be used to uniquely map the set of interactions on a document to the corresponding user. These interaction logs are very granular and include roughly 2000 unique commands.
%\rw{I'd be clear here that the logs are really granular - command level}
For a subset of these documents, we also have some numeric statistics on the content of these document (e.g.  \texttt{\#}words,  \texttt{\#}sentences,  \texttt{\#}charts, etc) that are logged as static snapshots at different time points.
Finally, for a yet smaller subset of documents, we have access to some statistics on typing traces that includes timing information on the duration of typing by different users with respect to a document. We do not have access to any keystroke-level data or the actual characters that were typed.

\subsubsection{Lifetime of Documents}
Four our purposes, the lifetime of a document ranges from its creation to the last user interaction with the document during our 3 month window. We find that the majority of documents in our collection have a short lifetime (less than 24 hours - See Figure \ref{LifetimeDist}).  

\begin{figure}[htb!]
\centering
\includegraphics[width=0.5\textwidth]{LifetimeDist.png}
\caption{Distribution of lifetime across all documents in our collection. Documents with lifetime shorter than 1 hour are removed \rw{why? can we say anything about the frequency of those? why they might have such a short lifetime?}.}
\label{LifetimeDist}
\end{figure}
\vspace{-1mm}

%\rw{I'd avoid using the word correlation unless we're going to report a correlation statistic such as Pearson (which we could/should?) - I'd prefer ``relationship''}
There is a relationship between the number of collaborators involved in a document and the lifetime of the document. Figure \ref{Lifetime_vs_numUsers} shows that the lifetime of documents has a non-decreasing trend as the number of authors increases ($r = 0.78, n = 20, p < 0.0001$). \bs{Pearson correlation statistics based on documents up to 20 users.}

\begin{figure}[hb!]
\centering
\includegraphics[width=0.5\textwidth]{Lifetime_vs_numUsers.png}
\caption{Distribution of lifetime across all documents in our collection (documents with lifetime < 1 hour removed \rw{again, why?}).}
\label{Lifetime_vs_numUsers}
\end{figure}
\vspace{-2mm}

\subsubsection{Preprocessing}
% old version is commented out.
We take two major preprocessing steps to prepare our log data for more robust analysis. In the first step we
address two issues with our logs: (1) Our dataset does not include any information on the content of documents and textual changes beyond a fine-grained set of commands capturing users' interactions with the writing application; and (2) these logged interactions are at a very fine-grained command level: we have over 2000 unique commands in our logs, each of which can be relatively sparse in its occurrence. 

To address this, we need to provide a mapping between low level users actions to more high level activities which begin to correspond to more meaningful writing behavior. 
% To this end, for a subset of the commands three independent annotators investigated the effects of each command to the document environment and used an activity label that objectively described this action. These sets of activity labels were then unified by resolving conflicts across annotators and finalizing a repository of activity labels. Finally, one of the annotators completed the groupings for the remainder of commands based on this repository. 

First, to develop initial categories of activities, a subset of all commands were reviewed by three annotators independently to identify the impact of applying those commands to the writing environment. The impact of a command was investigated based on widely accepted operations that change the content of a document (i.e., adding, editing and deleting) as well as commands that have no impact on the document content (e.g. viewing, navigating, communicating, etc).

The annotators then engaged in an iterative vetting process \footnote{Iterative vetting involves using the output of one stage to determine the next stage, incrementally reaching a final objective.} to group commands based on how they impact the document as well as the writing environment in general and refined the formed groups until no more groups were found. For example, all commands that result in adding some content (text, shapes, citations, etc) to the document are grouped together as \textit{Adding}, while commands that are only used for navigating throughout the document (e.g., NextHeader, GoToPreviousPage, etc) are grouped into \textit{Navigation} activity.
Since there is not much ambiguity in whether a specific command impacts the document content the agreement among the annotators was generally high. These sets of activity groups were then unified by resolving conflicts across annotators and finalizing a repository of activity categories. Finally, one of the annotators completed the groupings for the remainder of commands based on this repository.
%As a result, a taxonomy of 48 activity categories was created.
This process resulted in a set of 48 activity labels. These activity labels were then classified into 12 higher level activity categories that more closely correspond to writing activities. Figure \ref{CategorizingCommands} shows higher levels of this taxonomy. These high level groupings are sufficiently general and are supported by a variety of modern writing tools.
\vspace{-1mm}


\begin{comment}
We take two major preprocessing steps to prepare our log data for more robust analysis. In the first step we
address the issue that the logged interactions in our data are at a very fine-grained command level: we have over 2000 unique commands in our logs, each of which can be relatively sparse in its occurrence. 
\bs{I still believe as one novelty about our work is the fact that we are studying document authoring without having access to the textual content of the documents, it is worth elaborating on the process of getting from low level interaction logs to high level activities that correspond to writing behavior. So I'd like to put back a short description of this process by refining what I had written before.} \rw{logs no content seems like a shortcoming rather than an advantage - let's be clear on why we think this is an advantage}\\
%need to address two issues with this data: (1) We do not have access to the text of the documents and our only way of tracking the changes a user is applying to a document through the set of commands logged as users interactions with the Word UI in our dataset. (2) These commands are very fine grained and we have over 2000 unique commands in our logs which makes tracking the user's interaction with the writing tool very complex.
To address this, we provide a mapping between low level users actions to more high level activities which begin to correspond to more meaningful writing behavior. 
%Our main criteria for grouping different commands into a higher level category label is based on the impact of that command on the document. 
For example, our commands that result in adding some content (text, shapes, citations, etc) to the document are grouped together as \textit{Adding}, while commands that are only used for navigating throughout the document (e.g., NextHeader, GoToPreviousPage, etc) are grouped into \textit{Navigation} activity. This categorization was performed using three annotators. \rw{this raises questions about the specifics of the annotation process, instructions to annotators, inter-annotator agreement, disagreement resolution - we should add this}

%To this end, for a subset of the commands three independent annotators investigated the effects of each command to the document environment and used an activity label that objectively described this action. These sets of activity labels were then unified by resolving conflicts across annotators and finalizing a repository of activity labels. Finally, one of the annotators completed the groupings for the remainder of commands based on this repository. 

This process resulted in a set of 48 activity labels. These activity labels were then classified into 12 higher level activity categories that more closely correspond to writing activities. Figure \ref{CategorizingCommands} shows a subset of this taxonomy \rw{how was this this chosen? is it representative?}.
\end{comment}

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{commands2.pdf}
\caption{Placeholder for Categorizing Commands Figure.}
\label{CategorizingCommands}
\end{figure}
\vspace{-1mm}

\begin{comment}
\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{commands.pdf}
\caption{Placeholder for Categorizing Commands Figure.}
\label{CategorizingCommands}
\end{figure}
\end{comment}
\vspace{-1mm}
The second step of our preprocessing involved a principled way of reducing noise in our collection of documents by removing documents with very short lifetimes that do not provide enough interaction signals for studying document authoring behavior. To this end, we limited our analysis to documents with at least 2 users as they tend to correlate with longer lifetimes. \rw{we need to be very careful in how we justify this - it has implications for the generalizability of the findings} Further, we used 10 users as an upper bound since our survey data indicated that 98\% of shared documents that are written for work purposes involve between 2 and 10 collaborators.

\subsubsection{Final Dataset}
\label{FinalDataSet}
Our final dataset includes about 170k documents where the majority has 2 or 3 collaborators involved (78\% and 12\% respectively). Lifetime of documents in this final set are higher and more evenly distributed overall (Figure \ref{LifetimeDist_CW}).

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{LifetimeDist_CW.png}
\caption{Lifetime of collaborative documents in the preprocessed dataset.}
\label{LifetimeDist_CW}
\end{figure}
\vspace{-1mm}

% over a two weeks period from May 6, 2018 to May 19, 2018. The email Web client can be used on both desktop and mobile with multiple browsers. 
% Our sample consists of forty thousand active users who performed about 3 million actions during the two weeks period. Our sample included emails from enterprise users only. The logs do not contain the text of the email message, email headers or email search queries. The email log contains actions performed against messages with timestamps and other metadata. We limit our analysis to active users by excluding any user that interacts with less than 1\% of received email in the two week period
\subsection{Magnitude of Writing Activities Over Time} \label{Data:Catplots}

% We can now begin our investigation of how the interaction between writers and their corresponding documents changes over time. 
In order to be able to track these interactions over time we first segment the lifetime of each document into 10 equally sized segments and look at the magnitude of interactions at each of these segments.
\begin{comment}
\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{Catplot_CW_HD.png}
\caption{Distribution of Frequency of Writing Activities Over Stages of Document Evolution (Multi-author Documents). \rw{we should call these CAT plots in the caption too}}
\label{Catplot_CW}
\end{figure}
\end{comment}

\begin{figure*}[bht]
  \centering
  \subcaptionbox{Single vs Multi Author Docs\label{fig:SAD_MAD}}{
    \includegraphics[width=0.31\textwidth]{Catplot_SAD_MAD.png}
  }
  \subcaptionbox{Different Lifetimes\label{fig:MAD_Lifetimes}}{
    \includegraphics[width=0.31\textwidth]{Catplot_MAD_differentLifetimes.png}
  }
  \subcaptionbox{Different \texttt{\#} Collaborators\label{fig:MAD_numCollaborators}}{
    \includegraphics[width=0.31\textwidth]{Catplot_MAD_1W_2_5_10U.png}
  }
  \caption{Distribution of Frequency of Writing Activities Over Stages of Document Evolution (a) Single vs Multi Author Docs, (b) Multi Author Docs Different Lifetimes and (c) Multi Author Docs with Different \texttt{\#}Collaborators.}
  \label{fig:Catplots}
\end{figure*}

Figure \ref{fig:Catplots} shows how the level of users interactions with the writing application is changing over time. \bs{find a way to add in authors' Contributions Across Time (CAT).}\\
These activities are normalized by the total frequency of activities at the end of the lifetime of the documents. We can see an interesting pattern where there is a high level of activities at the very early and very late stages of document writing while the middle stages show a much lower interaction with the writing application overall.

Interestingly, even when we move away from single-author documents to multi-author ones with different number of collaborators involved (See Figure \ref{fig:SAD_MAD}), the overall pattern does not change. We also experimented with documents of different lifetimes (i.e. short (between 1 and 24 hours); medium (within a week); long (more than 2 months) - Figure \ref{fig:MAD_Lifetimes}), as well as different number of collaborators with the same lifetime (Figure \ref{fig:MAD_numCollaborators}) and noticed the same pattern persisted throughout.  

The progression of these writing activities over the document lifetime is interesting because it reflects different levels of interaction with the writing application at different stages. There is a notable difference at early and later stages of document authoring that could be attributed to the task management aspects of document writing and how authors distribute the workload over the course of the writing process. Another implication of this observation is in predicting the lifetime of documents by observing the changes in the rate of interactions between the users of a writing application and the writing environment. We revisit the problem of predicting the document's lifetime later in Section \ref{predictionSection}. 
%\rw{Mention here that we come back to this later in the doc} 

Please note that this CAT distribution can only be observed at the end of the document lifetime where we can compute the percentage of activities at different stages of the document evolution. That is, throughout the document evolution we can only capture the rate at which the interactions level is changing and compare it against previous snapshots of the document. 
%\rw{the ``That is'' seems to make a different point to the previous sentence}\bs{added 'only' to fix that?}

% The analysis of actions frequency over the lifetime of the documents showed an interesting pattern that persisted through documents with different lifetimes and different number of collaborators. These plots demonstrated a high level of activities in the first and last 10\% bucket with a low, flat activity level over the middle stages.

\subsection{Types of Activities in Early versus Late Stages}
\begin{figure*}[htb!]
\centering
\includegraphics[width=0.9\textwidth]{ActivityTypes_overTime.png}
\caption{Distribution of Types of Writing Activities Over Stages of Document Evolution.}
\label{ActivityTypeDist}
\end{figure*}
The next research question we investigated was whether our qualitative observations regarding the types of activities that writers do in earlier versus later stages can be observed in our large scale dataset of users interactions?

Recall that based on our survey responses outlining, structuring the document and drafting were among the early activities while proofing, collaborative activities, referencing and etc. were identified as later stage activities.

Reusing our lifetime segmentation of documents' activities we looked more closely at the types of activities that were observed in our logs and how they are distributed across these 10 segments. A subset of activities that correspond to the ones mentioned by our survey participants were used for this analysis. Figure \ref{ActivityTypeDist} demonstrates the distribution of these activities over these 10 stages of document evolution. These activities are ordered from left to right based on how early they are likely to be observed during the document evolution. \rw{Is that true? ``Pictures'' and ``Hyperlinks'' seems out of place then} %\cite{salas:calculus}, \cite{reid:scribe}, \cite{lamport:latex}.

The distribution of each of these activities over the 10 stages of document lifetime is normalized by their overall. The two peak of activities in the first stage (Stage 1) and last stage (Stage 10) is evident in these distributions as well. However, when comparing the likelihood of an activity between the first and the last stage we can see differences in the distributions of writing activities at the different stages. 
For example, activities such as interacting with HeaderFooter, Styles, Paragraph, and BulletsAndNumbers are more likely to be observed during the earliest stage of document authoring than the latest stages (e.g., 37\% vs 24\% for HeaderFooter; 34\% vs 23\% for styles and paragraphs). These activities correspond to initialing the overall structure of the document, outlining and early stages of drafting which involves creating and modifying lists and working them into paragraphs. A variety of advanced objects including Tables, Shapes, Equations and Charts are added and manipulated that are more likely to be observed throughout the middle stages with Tables and Shapes preceding Equations and Charts. 

\bs{email is sent regarding additional analysis to be done.}
%\bs{I just noticed the likelihood of observing Proofing in the early or late stage (30\% likely in Stages 1-2 vs 33\% likely in Stages 9-10) is not very different to call it a late stage activity as identified by our qualitative findings. One issue is that Proofing glump can include commands such as "IgnoreSuggestion" etc which could indicate the user doesn't want these suggestions but I don't have a breakdown of commands under this glumps while they are very easy to generate :( } \rw{either we do this analysis tomorrow if possible or we include this as a discussion point/limitation}\\
Among the later stage activities we can see improving the writing style (e.g., utilizing Synonym functionality) is more likely to be done at a later stage. Collaborative activities such as TrackChanges and Commenting are also happening towards the end of the document lifetime. 

\subsubsection{Distribution of First Activities.}
For each document in our dataset we also looked at the distribution of first activities of individual users as a proxy for the mode or intent behind attending to a document. To simplify this analysis we compared the distribution of the first activities of the first authors and the seconds authors of shared documents. That is the authors of a shared document were ordered by their time of their first activity and we collected the type of their first activity as well as all activities.

Contrasting the distribution of all activities by the first and the second writers of a shared document we do not see a a high variety. Overall Formatting, Adding and Modifying Content accounts for 22\%, 15\% and 15\% for both first and second authors. The main two distinctions are for Typing and Initiating Communication (e.g. adding a new comment) that accounts for 5\% and 0.7\% of second author's overall activities but only to 2\% and 0.4\% of first author's overall activities.  

Once we shift our focus to the first activities of the first and second authors at the time they first attend to a shared document, we start noticing differences in their intent and modes of writing. Our log based analysis indicated that the second authors are 7 times more likely to start their interaction with typing and 2.5 times more likely to start with adding non textual content (e.g. advanced objects) compared with the first authors (14\% vs 2\% and 10\% vs 4\% respectively). 
A similar trend is observed with second authors being two times more likely to start with editing activities (i.e. modifying content and formatting - 10\% vs 5\%). 
Finally, not only second authors initiate communication more than the first authors throughout the document lifetime, they are also three times more likely to attend to a shared document for the first with a communication intent (i.e. commenting and change tracking activities).   

\rw{There's been a lot in this section and a brief summary - 2-3 sentences would be helpful in wrapping it up and leading into the prediction task}

\begin{comment}
\begin{table*}[h]
\centering
\caption{Frequencies of different activities over 10 stages of document evolution normalized by total frequency of that activity. 
}\label{tbl-read-revisit}
%\vspace{-10px}
\begin{tabular}{ l | l l l l l l l l l l l}
  \hline
  Activity & Stage1 & Stage2 & Stage3 & Stage4 & Stage5 & Stage6 & Stage7 & Stage8 & Stage9 & Stage10 \\
  \hline
  Font		 & 0.004 & 0.021 & 0.001 & 0.017 & 0.038 & 0.015 & 0.139 & & & \\
  Pictures 	 & 0.054 & 0.005 & 0.011 & 0.014 & 0.008 & 0.086 & 0.096 & & & \\
  Paragraph 	 & 0.121 & 0.007 & 0.003 & 0.034 & 0.008 & 0.060 & 0.087 & & & \\
  BulletsAndNumber 	 & 0.054 & 0.003 & 0.003 & 0.008 & 0.004 & 0.0300 & 0.027 & & & \\
  Tables    & 0.054 & 0.003 & 0.003 & 0.008 & 0.004 & 0.0300 & 0.027 & & & \\
  Shapes    & 0.054 & 0.003 & 0.003 & 0.008 & 0.004 & 0.0300 & 0.027 & & & \\
  TrackChanges  & 0.054 & 0.003 & 0.003 & 0.008 & 0.004 & 0.0300 & 0.027 & & & \\
  HeaderFooter  & 0.054 & 0.003 & 0.003 & 0.008 & 0.004 & 0.0300 & 0.027 & & & \\
  Proofing      & 0.054 & 0.003 & 0.003 & 0.008 & 0.004 & 0.0300 & 0.027 & & & \\
  Synonym       & 0.054 & 0.003 & 0.003 & 0.008 & 0.004 & 0.0300 & 0.027 & & & \\
  Styles        & 0.054 & 0.003 & 0.003 & 0.008 & 0.004 & 0.0300 & 0.027 & & & \\
  Equations     & 0.054 & 0.003 & 0.003 & 0.008 & 0.004 & 0.0300 & 0.027 & & & \\ 
  Commenting    & 0.054 & 0.003 & 0.003 & 0.008 & 0.004 & 0.0300 & 0.027 & & & \\
  Bibliography  & 0.054 & 0.003 & 0.003 & 0.008 & 0.004 & 0.0300 & 0.027 & & & \\
  Hyperlinks    & 0.054 & 0.003 & 0.003 & 0.008 & 0.004 & 0.0300 & 0.027 & & & \\
  TableOf   & 0.054 & 0.003 & 0.003 & 0.008 & 0.004 & 0.0300 & 0.027 & & & \\
  FindReplace   & 0.054 & 0.003 & 0.003 & 0.008 & 0.004 & 0.0300 & 0.027 & & & \\
  Charts    & 0.054 & 0.003 & 0.003 & 0.008 & 0.004 & 0.0300 & 0.027 & & & \\
  InsertObject  & 0.054 & 0.003 & 0.003 & 0.008 & 0.004 & 0.0300 & 0.027 & & & \\
  \hline
\end{tabular}
\end{table*}

\end{comment}



==> sec.QuantitativeFindings.tex <==
\section{Quantitative Findings}
In our quantitative analysis we focus on quantifying how authors interact with the writing application over stages of a document lifetime.
%\rw{These questions should be formatted in the same way as those at start of Section 3}
Overall we found that writers distribute their writing activities
differently over stages of document authoring both in
terms of magnitude as well as types of these activities. The following two subsections describe these differences in detail.

%1. Are there differences in the magnitude of user's interaction at different stages of the document evolution?\\
%2. What types of writing activities are pertaining to earlier versus later stages of document evolution?
%\vspace{-1mm}
\subsection{Magnitude of Writing Activities Over Time} \label{Data:Catplots}
%\vspace{-0.5mm}
% We can now begin our investigation of how the interaction between writers and their corresponding documents changes over time. 
We first characterize a document's temporal stages by tracking the magnitude of author interactions with the writing application over a document's lifetime, hereinafter referred to as Contributions Across Time (CAT). To this end, we segment the lifetime of each document into 10 equally sized buckets and look at the magnitude of interactions in each of these segments.
\begin{comment}
\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{Catplot_CW_HD.png}
\caption{Distribution of Frequency of Writing Activities Over Stages of Document Evolution (Multi-author Documents). \rw{we should call these CAT plots in the caption too}}
\label{Catplot_CW}
\end{figure}
\end{comment}

\begin{figure*}[bht]
  \centering
  \subcaptionbox{Single vs Multi Author Docs\label{fig:SAD_MAD}}{
    \includegraphics[width=0.47\textwidth]{CAT_SAW_CW.pdf}
  }
  \subcaptionbox{Different Lifetimes\label{fig:MAD_Lifetimes}}{
    \includegraphics[width=0.47\textwidth]{CAT_MAD_DiffLifetimes.pdf}
  }
  \subcaptionbox{Different \texttt{\#} Collaborators\label{fig:MAD_numCollaborators}}{
    \includegraphics[width=0.47\textwidth]{CAT_DiffNumCollabs.pdf}
  }
  \caption{Distribution of frequency of writing activities over stages of document evolution (a) single vs multi author documents, (b) multi author documents with different lifetimes, and (c) multi author documents with different \texttt{\#}collaborators.}
  \label{fig:Catplots}
\end{figure*}

Figure \ref{fig:Catplots} shows these CAT distributions for different types of documents.
% There are 10 buckets over the lifespan of the document plus two additional buckets (pre and post) for before the document is created (0-operations) and after document editing ends (0-operations), yielding 12 points in Figure-4.  
%\bs{find a way to add in authors' Contributions Across Time (CAT).}\\
These activities are normalized by the total frequency of activities at the end of the lifetime of the documents. \footnote{The x-axis corresponds to the 10 buckets over the lifespan of the document plus two additional buckets (pre and post) for before the document is created (0-operations) and after document editing ends (0-operations), yielding 12 points in Figure-4.}  We can see an interesting pattern where there is a high level of activities at the very early and very late stages of document writing, while the middle stages show a much lower level of interaction with the writing application overall.

Interestingly, even when we move away from single-author documents to multi-author documents with a different number of collaborators involved (See Figure \ref{fig:SAD_MAD}), the overall pattern does not change. We also experimented with documents of different lifetimes (i.e., short [between 1 and 24 hours]; medium [within a week]; long [more than 2 months] - Figure \ref{fig:MAD_Lifetimes}), as well as different number of collaborators with the same lifetime (Figure \ref{fig:MAD_numCollaborators}) and noticed the same pattern persisted throughout.  

The progression of these writing activities over the document lifetime is interesting: there is a notable difference at early and later stages of document authoring that could be attributed to the task management aspects of document writing and how authors distribute the workload over the course of the writing process. Another implication is in predicting the lifetime of documents by observing the changes in the rate of interactions between the users of a writing application and the writing environment. We revisit the problem of predicting the document's lifetime in Section \ref{predictionSection}. 
%\rw{Mention here that we come back to this later in the doc} 

Please note that these CAT distributions can only be observed at the end of the document lifetime where we can compute the percentage of activities at different stages of the document evolution. That is, throughout the document evolution we can only capture the rate at which the interaction level is changing and compare it against previous snapshots of the document. 
%\rw{the ``That is'' seems to make a different point to the previous sentence}\bs{added 'only' to fix that?}
% The analysis of actions frequency over the lifetime of the documents showed an interesting pattern that persisted through documents with different lifetimes and different number of collaborators. These plots demonstrated a high level of activities in the first and last 10\% bucket with a low, flat activity level over the middle stages.
%\vspace{-2mm}
\subsection{Types of Activities in Early vs Late Stages}
%\vspace{-0.5mm}
\begin{figure*}[htb!]
\centering
\includegraphics[width=0.95\textwidth]{ActivityTypes_overTime_new.png}
\caption{Distribution of types of writing activities over stages of document evolution.}
\label{ActivityTypeDist}
\end{figure*}
%\vspace{-1mm}
%\bs{Sujay/Ryen - could you read 5.2?}

The next research question we investigated was whether our qualitative observations regarding the types of activities that writers perform in earlier versus later stages can be observed in our large scale dataset of user interactions.
Recall that based on our survey responses, outlining, structuring the document and drafting were among the early activities, while proofing, collaborative activities, referencing were identified as later stage activities.

Reusing our lifetime segmentation of authors' contributions we looked more closely at the distribution of different types of writing activities across these 10 segments.
% the types of activities that were observed in our logs and how they are distributed across these 10 segments. 
A subset of activities that correspond to the ones mentioned by our survey participants was used for this analysis. Figure \ref{ActivityTypeDist} demonstrates the distribution of these activities over these 10 stages of document evolution. These activities are ordered from left to right based on the difference between their shares in Stages 1 and 10 to reflect how early they are likely to be observed during the document evolution. 
%\rw{Is that true? ``Pictures'' and ``Hyperlinks'' seems out of place then} %\cite{salas:calculus}, \cite{reid:scribe}, \cite{lamport:latex}.

The distribution of each of these activities over the 10 stages of document lifetime is normalized by their overall frequency. Note that for each of the activity types, stages 1 and 10 are the most prominent stages in which they occur, which reflects the results from the CAT plots.
%The two peaks of activities in the first and last stage (stages 1 and 10 in the CAT distributions) is evident in these distributions as well. 
However, when comparing the likelihood of a writing activity between the first and the last stage we can see variations across activities. 
For example, activities such as interacting with HeaderFooter, Styles, Paragraph, and BulletsAndNumbers are more likely to be observed during the earliest stage of document authoring than the latest stages (e.g., 37\% vs 24\% for HeaderFooter; 34\% vs 23\% for styles and paragraphs). These activities correspond to setting up the overall structure of the document, outlining and early stages of drafting which involves creating and modifying lists and working them into paragraphs. A variety of advanced objects including Tables, Shapes, Equations and Charts are added and manipulated throughout the middle stages, with Tables and Shapes preceding Equations and Charts. 

%\bs{email is sent regarding additional analysis to be done.}
%\bs{I just noticed the likelihood of observing Proofing in the early or late stage (30\% likely in Stages 1-2 vs 33\% likely in Stages 9-10) is not very different to call it a late stage activity as identified by our qualitative findings. One issue is that Proofing glump can include commands such as "IgnoreSuggestion" etc which could indicate the user doesn't want these suggestions but I don't have a breakdown of commands under this glumps while they are very easy to generate :( } \rw{either we do this analysis tomorrow if possible or we include this as a discussion point/limitation}\\
Among the later stage activities we can see improving the writing style (e.g. finding Synonyms) is more likely to be a later stage activity (26\% vs 20\%). Collaborative activities such as TrackChanges and Commenting are also likely to happen towards the end of a document's lifetime.
Interestingly interacting with Proofing and Spelling functionalities are 11\% and 6\% more likely to happen at the latest stage, while Grammar related interactions seem to be middle stage activities. Finally, once we examine specific proofing commands we see some evidence of \textit{copy-editing mode} that seems to be more likely in later stages. For example, 28\% of all occurrences of NextMisspelling command, representing an author sequentially navigating through spelling suggestions by the writing tool, was observed at the latest stage (vs 22\% during the first stage).  
%\vspace{-2mm}
%However, once we examine the appearance of specific proofing-related commands we notice an interesting contrast between spelling (21\% vs 27\%) and proofing (20\% vs 31\%) related actions and interactions with grammar commands.
% Bahar: StatusSpellCheck command seems interesting only if we knew exactly what it represents! 
% distribution of this command:
\begin{comment}
StatusSpellCheck
20.66413558
6.556986171
5.128205128
4.920949342
4.91911522
4.91911522
5.49594659
6.426763508
8.45805363
32.51072961
\end{comment}
\subsubsection{Distribution of First Activities.}
For each document in our dataset we also looked at how activities differ between authors that start work on the document at an earlier or later stage. For this purpose, we ordered the authors of a shared document by the time of their first activity in the document and we collected the type of their first activity as well as the set of all their activities.
%For each document in our dataset we also looked at the distribution of first activities of individual users as a proxy for the mode or intent behind attending to a document. To simplify this analysis we compared the distribution of the first activities of the first authors and the second authors of shared documents. That is, the authors of a shared document were ordered by the time of their first activity and we collected the type of their first activity as well as all activities.
Contrasting the distribution of activities by the first and second authors of a shared document we do not see a high variation. Overall, Formatting, Adding and Modifying Content accounts for 22\%, 15\% and 15\% for both first and second authors. The main two distinctions are for Typing and Initiating Communication (e.g., adding a new comment) that accounts for 5\% and 0.7\% of second author's overall activities but only to 2\% and 0.4\% of first author's overall activities.  

Once we shift our focus to the first activities of the first and second authors at the time they first attend to a shared document, we start noticing differences in their intent and modes of writing. Our log based analysis indicated that the second authors are $7\times$ more likely to start their interaction with typing and $2.5\times$ more likely to start with adding non textual content (e.g., advanced objects) compared with the first authors (14\% vs 2\% and 10\% vs 4\% respectively). 
A similar trend is observed with second authors being two times more likely to start with editing activities (i.e., modifying content and formatting - 10\% vs 5\%). 
Finally, not only do second authors initiate communication more than the first authors throughout the document lifetime, they are also three times more likely to attend to a shared document for the first time with a communication intent (i.e., commenting and change tracking activities).   

%\rw{A brief summary - 2-3 sentences would be helpful in wrapping it up and leading into the prediction task.} \bs{I'll add this once the paper is fit to length.}

%\el{I would consider adding a discussion here, and then concluding the discussion with one remaining question is whether it is feasible to create stage-specific tools. Then I'd go on to Predicting the stage of a document.}
%\vspace{-1mm}
\subsection{Summary of Findings}
%\bs{needs refinement} 
From our qualitative data, we find that authors have a perception of stages or phases in the writing process and that these stages represent an ordering in the creation of a document -- from ideation through creation to refinement. Our quantitative data reflects this partially ordered approach to document creation through changes in both the magnitude of and types of interactions that occur over a document's lifetime.
% Synthesizing findings from both qualitative and  quantitative data, we find both that authors have a perception of stages of writing; and that these stages are reflected in changes in both the magnitude of and types of interactions over the document's lifetime. 
%While  that resonates with an overarching temporal ordering while it is also reflected in the changes in the magnitude and types of interactions with the writing tool over a document's lifetime. 
%and that the magnitude and types of interactions with the writing environment changes over a document's lifetime, correlating with the idea that different activities are correlated with different stages. 
Further, authors in our qualitative study welcome the idea of stage-appropriate writing assistance. They highlight varied goals and activities to which assistance can be tailored at different stages. Alongside the potential for stage-specific assistance, previous work has noted the importance of stage-appropriate behavior during collaborative tasks \cite{gutwin2002}, and therefore stage-aware tools have the potential to foster improved collaboration. 
%Complementary to this, our large scale interaction logs quantify the likelihood of observing a subset of these writing activities in different stages.
%Finally, while modes of writing was qualitatively identified as a relevant aspect of stages of writing, our interaction logs confirmed there are differences in the modes of authors attending to a shared document at different stages.  

In summary, implications of the synthesis of our qualitative and quantitative data is that \begin{enumerate*} \item there exists a perceived benefit to stage-specific writing assistance \item we observe different activities at different stages of the document lifespan, and \item stage awareness mechanisms can communicate to collaborators the current state of the document, which can aid in on-boarding of new collaborators and in appropriate behaviors during collaboration \cite{gutwin2002} \end{enumerate*}. However, to effectively design interfaces to support stage-specific writing tasks and to communicate stages, one open question remains: Can we predict the stage of writing given observation of user actions? To explore this last research question, we present a study in the next section assessing the feasibility of
stage-identification.
\begin{comment}
\section{Discussion}

My random musings on what might go in here.
\begin{enumerate}
    \item Examining both our qualitative and our quantitative study data, we see that writers have a perception of stages of writing and that tool use changes over a documents lifetime, correlating with the idea that different activities are correlated with different stages. Further, writers in our qualitative study welcome the idea of stage-appropriate interaction with writing tools. Can include editing features, discourse guidance (e.g. Gutwin) ...
    \item I'm a bit worried that stages may not be linear to the user but that the way the quantitative data was done makes them seem linear. So the question becomes can you map, somehow, activities onto stages, or correlate between this linearity and lifetime? I think an argument can be made that stages are primarily linear, even if they aren't purely linear, in many cases. Can you use shorter document lifespans to have a better notion of individual stages? Are there unistage documents (e.g. documents where the writer writes but never edits, documents where the writer copies everything in and just revises, documents where neither is done but it is shared).  See if the argument can be tightened between temporal stages and cognitive stages, or that somehow these can be shown to be near equivalents.
    \item Conclude by saying that there seems to be, therefore, an significant potential benefit to stage-specific writing tools, but that one question remains: are they feasible? To explore this, we describe a last feasibility study that shows that we can predict stage from operations.
    
\end{enumerate}
\end{comment}

==> sec.RelatedWork.tex <==
\section{Related Work}
%Intelligent writing assistance can be viewed as a systematic way of providing recommendations regarding different aspects of writing (e.g., spelling, grammar, writing style, structuring, etc) with a goal of improving the document quality.

%In the domain of recommender systems, there has been a shift towards context-aware recommendation \cite{adomavicius2011, shi2014, hariri2013} that aims to leverage contextual information to improve the quality of personalized services. These systems are shown to generate more relevant recommendations by adapting them to the specific contextual situation of the user. They can be characterized by two main stages: defining context \cite{cao2010} and incorporating that context \cite{adomavicius2011}. 

%Despite the wide-spread use of context aware intelligent systems in many domains (e.g. conversational search, travel planners, calendar-aware email recommendation, etc.), modern writing tools often ignore the notion of writers' ``situated actions'' \cite{schuman1987} beyond the word or sentence level textual content \cite{heidorn2000}.

% Although there is no universal agreement on the precise definition of context, one of the most commonly used definitions, proposed by Abowd et al \cite{abowd1999}, defines context as ``any information that can be used to characterize the situations of an entity,'' and by entity they mean ``a person, place or object that is considered relevant to the interaction between a user and an application, including the user and applications themselves''.

% Applying this definition to writing tasks there are still many ways one can define which context is relevant for supporting a user during their interaction with the writing tool: the context of the writer? the context of the writing task? the context of the interaction? or the context of the situation?

% In this paper we motivate the notion of ``stage of a document under development'' or ``the stage of document evolution'' as one type of relevant situated context to leverage for providing intelligent writing assistance. Our rationale is that it incorporates some of the writer's mental model of the document as well as a set of interactions (or writing activities) that are affiliated with that stage of document evolution.

%The rest of this section reviews three main areas of past research that motivates the \textit{stage of document evolution} as one type of relevant situated context to leverage for providing intelligent writing assistance.

There are several areas of research related to stages of document authoring and intelligent writing assistance. We review them in what follows and highlight differences to our work.

\paragraph{Writing Process}
%\subsection{Writing Process}
A number of papers have previously investigated the process of writing, both as an individual task and as a collaborative endeavor.
%Extensive research has been conducted into how people write individually and in groups. From this research a number of theories of  writing have been developed. This has in turn inspired the development of computer tools to support various tasks and activities involved in the writing process.
Some studies of individual writing focus largely on text itself. These characterize writing as an ``outline-draft-edit'' cycle, assuming that ``meaning'' is assembled in the user's mind first and then articulated in text \cite{mitchell1996}.
Other studies adopt the \textit{process} view of writing instead, basing themselves on cognitive process models~\cite{freedman1987} for problem solving that involve sequences of activities, 
%with in the late 1970s \cite{freedman1987} with the development of cognitive process models of composing.
%Writing was thought of as a process of problem solving involving a sequence of activities,
including setting goals, planning, organizing, transcribing and editing.
Fitzgerald \cite{fitzgerald92} presents a comprehensive overview of early approaches to to the study of writing. She identifies three models of writing: the Stages Model \cite{rohman1965}, the Problem-solving Model \cite{flower1984}, and the Social Interaction Model \cite{nystrand1989}. 
%Although these models might be appearing to be in conflict,
These models can be seen as complementary: the Stages Model focuses on the construction of the text itself, the Problem-solving Model steps back and looks at the writers in context% and aims at incorporating the mental processes involved in the writing process.
and, the Social Interaction Model characterizes writing as a negotiation between the writer and the reader. %and addresses the social aspects of writing.
While there is no single theory or model of the writing process \cite{greer2016}, the Flower and Hayes model \cite{flower1981} is one of the more widely accepted ones. It considers writing as a series of cognitive processes.
Through a think-aloud study they show that the writing process involves three main sub-processes: planning, translating and reviewing.
Models of writing processes have been evaluated observationally in different ways, %both during and after the writing process, using observations,
using -- for example -- video analysis \cite{xu2014}, thinking-aloud methods (e.g. \cite{flower1981}) and retrospective interviews (e.g., \cite{posner1992}), mostly conducted in small scale and controlled settings.
%\bs{add references to each of these areas.} 
Most of these studies rely on directly observing the writers and are mostly conducted in small scale and controlled settings. 

There has been some effort on using keystroke logging to measure writing processes during typing (e.g., \cite{conijn2019, tillema2011, steck2018}). %These efforts have a great potential in providing real-time, fine-grained information on writers' unfolding typing process during text composition that can scale beyond traditional think-aloud and observational studies. 
For example, Conijin et al. \cite{conijn2019} investigated which and how keystroke features 
%are affected by differences in cognitive load across writing tasks that 
could provide insights into detecting the high level writing processes such as planning, translating and reviewing as the writers are typing.

\subsection{Revision Research}
The concept of \textit{revision} is inseparably connected with the writing process. Revision was defined as ``making any changes at any point in the writing process. It involves identifying discrepancies between intended and instantiated text, deciding what could or should be changed in the text and how to make the desired changes. These changes may or may not affect the meaning of text, and they may be minor or major'' \cite{fitzgerald1987}.

Recognizing the importance of rewriting and the revision process in successful writing, extensive research was conducted to understand and utilize revisions. Faigley and Witte \cite{faigley1981} showed that expert writers revise in ways different from inexperienced writers. These findings motivated a line of work that studied the relationship between revisions and text quality.

Revision research broadly falls into three categories: revision extraction, revision categorization and revision classification.

Several fields are involved in research on revision, the most relevant to our work is research conducted in the domains of education and computer science. 
In the education domain, analysis of revisions has typically relied on resource-intensive manual observation of students' essay writing practices in classrooms, and coding of writing behaviour, as well as grading the textual products of revisions. The main motivation behind this line of work is to analyze the relationship between revision and either text quality (e.g., \cite{sommers1994}) or the learning effect (e.g., \cite{murray1980}).

With the increasing popularity of different online writing tools (e.g. GoogleDoc) and text production communities (e.g. Wikipedia) numerous repositories of documents' revisions history became widely available. These repositories provided a great opportunity for studying the types and effectiveness of revisions.  
Specifically, differences between revisions contain valuable information for modelling document quality or extracting users' expertise and can additionally support various natural language processing (NLP) tasks \cite{yang2017}.

Especially Wikipedia article revision histories have been used to develop writing support techniques such as sentence compression \cite{yamangil2008}, lexical simplification \cite{yatskar2010}, information retrieval \cite{aji2010}, textual entailment recognition \cite{zanzotto2010}, language bias detection \cite{recasens2013}, spelling errors and paraphrases \cite{zesch2012, max2010}.
\bs{Revision research was included in RW to provide an overview of the state-of-art NLP systems that can provide support during writing. But it has to be re-positioned so we end up with the 3 sub-sections that contribute to the concept of ``stages of document writing''.}

\subsection{Decomposing the Writing Process}
The cognitive process model of writing \cite{flower1981} considers writing as a series of cognitive processes that are distinctive and hierarchical which enables writers to construct highly personal, idosyncratic and complex workflows \cite{teevan2016}.

The complexity of the writing process requires authors to coordinate multiple and often competing writing processes \cite{alamargot2001, alamargot2009, flower1981} 
% (Alamargot & Chanquoy, 2001; Alamargot & Fayol, 2009; Becker, 2006; Flower & Hayes, 1980; Hayes, 2012; Hayes & Flower, 1980).
These processes compete for a writer's attention which can lead to problems in balancing the complexities of managing many concurrent processes \cite{kellogg1988, greer2016}.

In writing, high level processes such as planning and reviewing are considered to have a high demand as they require high levels of attentional control [References]. Especially non-expert authors have been shown to utilize strategies to reduce the cognitive load by \textit{decomposing} the writing task and transforming it into smaller, more manageable subtasks and phases \cite{greer2016}. Separately addressing specific subgoals, such as idea generation, organization of ideas, revision of content, or editing for language, can help novice writers improve the quality of their work by focusing successively on different aspects of the writing process \cite{graham2012, kellogg1988, limpo2013}.

%Decomposing writing by different rhetorical categories can ease the cognitive demands of different processes \cite{greer2016}. For example, addressing specific subgoals, such as idea generation, organization of ideas, revision of content, or editing for language, can help novice writers improve the quality of their work by focusing successively on different aspects of the writing process \cite{graham2012, kellogg1988, limpo2013}. %(Fayol, 1999; Graham & Harris, 2012; Harris & Graham, 2009; Harris, Graham, & Mason, 2006; Kellogg, 1987; Limpo & Alves, 2013).

Kellogg \cite{kellogg1988}
%, as a pioneer researcher in the areas of attentional overload and writing performance, 
conducted experiments that showed decomposing the writing task at hand by a document's developmental stages, such as pre-writing, writing and post-writing is valuable because it scaffolds the work, prompts thoughtful engagement with tasks people would normally skip, and eases cognitive load \cite{teevan2016}.

\subsection{Workspace Awareness}
\bs{This section should talk about the awareness of document stage as a concept that is reflected in the mental model of writers. [will be re-written]}\\
The final area of past work that motivates leveraging the stage of document evolution as context for providing writing support is the notion of workspace awareness that is more prominent in a collaborative scenario where a group performs different tasks in a shared environment. Previous researchers have defined awareness as knowledge created through interaction between an agent and its environment. That is, awareness is knowledge about the state of an environment bounded in time and space. As well, environments change over time, so awareness is knowledge that must be maintained and kept up to date.

In the context of writing tasks, and more specifically collaborative writing, the shared document represents the workspace and can be considered an externalization of the task at hand. 

Gutwin and Greenberg \cite{gutwin2002} motivate the importance of workplace awareness for collaborative scenarios which can reduce effort, increase efficiency and reduce errors for the activities of collaboration.
For example, awareness of the stage of document helps with coordination of and suggesting the ways new collaborators can contribute and assist the writing process.

Assisting others with their local tasks is an integral part of collaboration and one that also benefits from workspace awareness. Awareness in this situation is useful because it helps people determine what assistance is \textit{required} and what is \textit{appropriate}.

\bs{To be completed and re-phrased.}



==> sec.RelatedWork_long.tex <==
\section{Related Work}
\begin{itemize}
    \item Seminal Theories of Writing Process and Related Taxonomies
    \item Analyzing textual changes using Documents versions history to support a variety of NLP tasks (mostly done on Wikipedia articles) + EMNLP paper
    \item Versions of Students Essays in classroom to understand what patterns lead to higher quality writing and support students with their writing tasks (focus on education)
    \item recommender systems
    \item Workspace Awareness and Collaborative Writing Support
\end{itemize}

\subsection{Writing Process}
Extensive research has been conducted into how people write individually and in groups. From this research a number of theories of  writing have been developed. This has in turn inspired the development of computer tools to support various tasks and activities involved in the writing process.

The early studies of individual writing focused largely on \textit{product} or the text itself. The standard attitude towards the writing process characterized it as an ``outline-draft-edit'' cycle. This assumes that meaning is clarified in the head first and then articulated clearly to express the meaning in text (Mitchell, 1996).

There was a shift to \textit{process} in the late 1970s (Freedman, Dyson, Flower and Chafe, 1987) with the development of cognitive process models of composing. Writing was then thought of as a process of problem solving involving a sequence of activities, including setting goals, planning, organizing, transcribing and editing.

Fitzgerald \cite{fitzgerald92} presented a comprehensive overview of early approaches to to the study of writing. She identifies three models of writing: the Stages Model \cite{rohman1965}, the Problem-solving Model \cite{flower1984}, and the Social Interaction Model \cite{nystrand1989}. 
Although these models might be appearing to be in conflict, they can in fact be seen as complementary, providing different perspectives on the same problem. The stages model focuses on the construction of the text itself, the problem solving model steps back and looks at the writers in context and aims at incorporating the mental processes involved in the writing process. Finally, the social interaction model characterizes writing as a negotiation between the writer and the reader and addresses the social aspects of writing.

While writing as a process resists being encapsulated in a single theory or model \cite{greer2016}, the Flower and Hayes model \cite{flower1981} is one of the more widely accepted ones, which considers writing as a series of cognitive processes.  Through a think-aloud study they show that the writing process involves three main sub-processes: planning, translating and reviewing.

Writing processes have been measured in different ways, both during and after the writing process, using observations, video analysis (e.g., \cite{xu2014}), thinking-aloud methods and retrospective interviews (e.g., \cite{posner1992}).
\bs{add references to each of these areas.}

\subsection{Revision Research}
A related concept that is inseparably connected to the writing process is \textit{revision}. Revision was defined as ``making any changes at any point in the writing process. It involves identifying discrepancies between intended and instantiated text, deciding what could or should be changed in the text and how to make the desired changes. These changes may or may not affect the meaning of text, and they may be minor or major'' \cite{fitzgerald1987}.

Recognizing the importance of rewriting and the revision process in successful writing, extensive research was conducted to understand and utilize revisions. The seminal work of Faigley and Witte \cite{faigley1981} showed that the expert writers revise in ways different from inexperienced writers. These findings motivated a line of work that studied the relationship between revisions and text quality.

Revision research can be broadly characterized as three areas of research: revision extraction, revision categorization and revision classification.

Several fields are involved in research on revision, each one with a different scope. Among them, the most relevant to our work is research conducted in the domains of education and computer science. 

In the education domain, analysis of revisions has typically relied on resource-intensive manual observation of students' essay writing practices in classrooms, and coding of writing behaviour, as well as grading the textual products of revisions. The main motivation behind this line of work is to analyze the relationship between revision and either text quality (e.g., \cite{sommers1994}) or the learning effect (e.g., \cite{murray1980}).

With the increasing popularity of different online writing tools (e.g. GoogleDoc) and text production communities (e.g. Wikipedia) numerous repositories of documents' revisions history became widely available. These repositories provided a great opportunity for studying the types and effectiveness of revisions.  

Specifically, differences between revisions contain valuable information for modelling document quality or extracting users' expertise and can additionally support various natural language processing (NLP) tasks \cite{yang2017}.

The main motivation behind these approaches, primarily using Wikipedia articles revisions histories, is developing tools to support writers. For example, a variety of NLP tools were developed for supporting different tasks such as sentence compression \cite{yamangil2008}, lexical simplification \cite{yatskar2010}, information retrieval \cite{aji2010}, textual entailment recognition \cite{zanzotto2010}, language bias detection \cite{recasens2013}, spelling errors and paraphrases \cite{zesch2012, max2010}.

\subsection{Decomposing the Writing Process}
The cognitive process model of writing \cite{flower1981} considers writing as a series of cognitive processes that are distinctive and hierarchical which enables writers to construct highly personal, idosyncratic and complex workflows \cite{teevan2016}.

However, there is a body of past research that shows decomposing writing by different rhetorical categories can aid the process and ease the cognitive demands of different processes \cite{greer2016}. 

In facts, writers, and more particularly the non-expert authors, are shown to use strategies that reduce the cognitive load of different mental processes involved. These strategies \textit{decompose} the complex task of writing and transform it into smaller, more manageable subtasks and phases \cite{greer2016}.

Kellogg \cite{kellogg1988}, as a pioneer researcher in the areas of attentional overload and writing performance, conducted experiments that showed decomposing the writing task at hand by a document's developmental stages, such as pre-writing, writing and post-writing is valuable because it scaffolds the work, prompts thoughtful engagement with tasks people would normally skip, and ease cognitive load \cite{teevan2016}.
\subsection{Contextual Recommendation}
Context-aware recommendation
systems (Shi et al., 2014; Hariri, Mobasher, and Burke, 2013) aim to leverage contextual information to improve the quality of personalized services. They can be characterized by two main stages: defining context (Cao et al., 2010) and incorporating that context. 
Incorporation of context can further be classified into three groups: pre-filtering,
post-filtering and contextual modeling (Adomavicius and Tuzhilin, 2011). Various approaches have been proposed to facilitate contextual recommendations for real world application.

These include news recommendations via contextual bandits (Li et al., 2010) or time-varying bandits (Zeng et al., 2016), context-aware point-of-interest recommendations (Yuan et al., 2013; Yao et al., 2015; Zhao et al., 2019), calendar-aware email recommendations (Zhao et al., 2018), sequential item recommendations (Hidasi et al., 2016; Tang and Wang, 2018; Yu et al., 2019), and contextual travel recommendations
(Kiseleva et al., 2016).



==> sec.StageAwareAssistance.tex <==
\section{Stage-aware Writing Assistance} 
Our main research question is to investigate whether providing writing assistance that is tailored to the current stage of a document development is beneficial to the writers of that document.
To this end we need to better characterize two different aspects of \textit{stage-aware writing assistance}: 
\begin{enumerate}
    \item \texttt{Characterizing the Stage of a Document:} How are the stages of document evolution perceived by the writers?
    \item \texttt{Characterizing the Writing Assistance:} What writing assistance is beneficial at different stages of document evolution?
\end{enumerate}

% There are many open questions in this space including how common writing documents at the workplace is, what support is needed, what are the expectations of an intelligent writing tool and whether there is a need for tailored support at different stages of writing?

To address these two questions, we began by conducting a survey at a large technology company with a range of close-ended as well as open-ended questions. 
% Most research on the writing process has been carried out in the context of education. Thus, little focus has been put on the particularities which arise when the writing process is carried out by information workers who need to write documents as a part of their daily routine at the workplace.
The survey data helped us understand how enterprise workers approach the writing of a document, how the stages of document authoring are perceived by them and what the expectations are for types of writing assistance at these stages.

\subsection{Survey}
We distributed a survey within a large technology company and collected 175 responses (completion rate: 70\%). 
Our survey started with a section on demographics including Job roles, number of current projects, team size, etc. The next section involved different questions regarding writing documents at the workplace which helped us verify whether writing documents at the workplace is a common practice, what tools are frequently used for writing documents and how often these documents involve other collaborators as well.

Respondents came from a diverse set of roles ranging from product managers and software developers to sales people and administrative assistants, the majority have been working at this company for more than 5 years (63\%).  Multi-tasking on different projects was a common trend among them, with 75\% working on at least 3 projects.
\subsection{General Findings}
%Our survey data confirmed that writing documents is very common at the workplace. 
87\% of our respondents mentioned they do need to write documents as a part of their work routine. They use a wide range of writing tools including Microsoft Word Desktop Client (89\%) and Online Client (49\%), followed by Notepad / Notepad++ (19.3\%), OneNote (16\%), Overleaf / Sharelatex (11.1\%), Google Docs (8.2\%), etc.

Collaboration on these documents was also a common theme among our participants with the majority (74\%) collaborating on at least 25\% of their documents.
Despite the commonality of collaborative writing, a closer examination of the qualitative responses (discussed below) indicated that the need for tailored support in different stages of document authoring is associated with both Single Author Writing (SAW) and Collaborative Writing (CW) scenarios. 
%While some of the participants talked about multi-author scenarios, the majority of responses could be applied to either of these scenarios. 
% Single author Writing (SAW) is defined as writing conducted by one individual that involves planning, drafting and reviewing (Lowry et al., 2004) Collaborative Writing (CW) builds on single-author writing by involving multiple people, thus increasing the complexity of the writing process (Galegher and Kraut, 1994).
\begin{quote}
\textit{``in and ideal scenario I would just do some sort of content dump to the system and the system structures this text. So that I don't have to think about paragraphs, sections, where to put what etc. And then in later stages I want help with how to nicely formulate things. That's not only in a collaborative setting though.''} [P10]
\end{quote}
As a first step towards understanding whether or not there is a need for different types of support at different stages of document evolution, in the next segment of our survey 
%included a series of questions to gauge real users perceptions and attitudes towards this concept. More formally, 
the participants were asked \textit{``Should an intelligent writing assistant provide different types of support at different stages of writing in the document?''} with a binary Yes / No response type.

Over 70\% of our participants expressed a need for different types of support at different stages of writing. The follow up open-ended questions to elaborate on their rationales for their response to this initial question revealed how these stages are perceived by the participants and that what support is needed at these stages. 

The responses to these questions were all analyzed using affinity diagramming. Data was initially clustered using open coding producing
19 clusters. Clusters were then analyzed using axial coding to identify overall themes in the data. We found that saturation for our
qualitative data occurred approximately after 80 participants, no
new clusters of information were identified. However, we continued
to cluster these responses for the remaining participants, particularly
attuned to data that might expand our clusters or add nuance to
our analysis. These clusters resulted in four broad themes, corresponding to different notions of the stage of a document as perceived by our participants and the utility of different types of writing assistance based on these stages.

The following three subsections elaborate on three different perceptions of a document's stage and the final subsection describes a different implication of awareness of the stage of a document that is essential for more effective collaboration over writing documents.

% (1) Supporting Early versus Later Stages of Document Evolution; (2) Supporting different phases of writing; (3) Supporting different modes or intents of writing; and (4) Awareness of Stage of Document is essential both for the intelligent System and the collaborating writers. We describe more details about these themes in the following subsections.

% better characterization of the

\begin{comment}
\subsection{Stage-based Support for both SAW and CW}
%Writers require different support at different stages of writing both in SAW and CW scenarios.

Single author Writing (SAW) is defined as writing conducted by one individual that involves planning, drafting and reviewing (Lowry et al., 2004)
Collaborative Writing (CW) involves multiple people, thus increasing the complexity of the writing process (Galegher and Kraut, 1994).

%While the complexity of CW scenarios is generally more amplified relative to SAW scenarios, 
A qualitative analysis of these survey responses indicated that the need for tailored support at different stages of writing is not only desirable for CW settings: the majority of responses are applicable to either of these scenarios. 
\begin{quote}
\textit{``in and ideal scenario I would just do some sort of content dump to the system and the system structures this text. So that I don't have to think about paragraphs, sections, where to put what etc. And then in later stages I want help with how to nicely formulate things. That's not only in a collaborative setting though.''} [P10]
\end{quote}

In unpacking the quote above we also see a time-based notion of stages of document writing that is further discussed in the following subsection.
\end{comment}

\subsection{Supporting Early versus Late Stages of Document}
The Stages Model of Writing \cite{rohman1965} focuses on the evolution of the text as an external by-product of the writing where the main three stages of pre-writing, writing and rewriting are separated in time. While more recent models (e.g. Flower and Hayes's model \cite{flower1984}) argue that a more realistic model of writing needs to focus on the mental processes involved in the writing process and that these mental processes are interleaved, hierarchically embedded and are not executed in a linear order, these models are indeed complementary and are not in conflict (Mitchell, 1996). 

%In fact, once we shift our view to the document as the by product of this process we can see some time based ordering of these high level stages of document evolution. 

%This view was shared amongst many of our participants who referred to these stages as early versus later stages of document writing.

Our participants perceived the early stages of writing to be highly focused and many participants expressed a desire for fewer interruptions and fewer system suggestions and notifications during these stages, particularly about minor fixes and improvements. 

%\advance\leftmargini 0.05em
\begin{myquote}{0.2in}
\textit{``I want fewer interruptions when i am focusing on adding content early in the document writing process.''} [P11]\\\\
\textit{``As someone who primarily writes documents in LaTeX, I like the ability to focus on writing the content without having to worry about formatting. Then only once the content is put down do I go back and tweak the look of the document. This allows me to focus on different aspects of the documents at different stages.''} [P12]\\\\
\textit{``Notifying me of grammar and spelling errors when I'm trying to get my thoughts out is really just a distraction. I prefer when these suggestions are made at a later editing stage.''} [P40]
\end{myquote}
The qualitative analysis of these responses indicated that participants can associate different phases of writing including Planning, Outlining and Early Drafting to \textit{Early Stages of Writing}. 

Participants discussed a variety of activities in earlier stages of writing which revealed the types of support that are the most appreciated in these early stages. Among them, outlining and deciding on the structure of the document as well as searching for relevant content were perceived as early stage activities. 
\begin{myquote}{0.2in}
    \textit{``Brainstorming and scope defining support \textbf{early on} that helps develop a basic outline and framework. It would be great for a writing assistant to help with the `starting from nothing' phase.''} [P98]\\\\
    \textit{``The needs at different stages may be very different. E.g. for structural changes, they better take place as \textbf{early} as possible; while for minor fixes or suggestions, they can come \textbf{later} when the body of text is by and large stable.''} [P64]\\\\
    \textit{``When \textbf{getting started}, Outline or Structure help is needed; \textbf{Later on} in the process, Editing, fact checking, adding references type of help is needed.''} [P84]\\\\
    \textit{``\textbf{Early:} Focus and scope - needed at the beginning to understand what to write about and how much; this is often org dependent and the ability to create org-specific templates and help advice would be amazing.  \textbf{Mid:} Content analysis and comparison, to highlight style and completeness differences in different areas.  \textbf{Late:} Advice on structural features and cleanups that can save time and improve accessibility.''} [P219]\\\\
    \textit{``Would be great to enter some notes and have an outline constructed. \textbf{Later} it would be great to have research done for me if I need a supporting quote or need a chart from another document. \textbf{Finally} it would help to have suggestions for alternatives to overused words.''} [P57]
\end{myquote}
Similarly, participants described a variety of activities that are not crucial to earlier stages of writing, for those activities system support can be perceived as \textit{distracting}, \textit{annoying} or \textit{not necessary}.
Overall, minor fixes, proofing and grammar fixes, collaborative activities such as commenting and change tracking are perceived as not helpful nor appreciated during early stages of document evolution.
\begin{myquote}{0.2in}
    \textit{``Different actions and needs are required for each stage of writing; i.e. there is no need to suggest spacing and layout changes when I've just started writing down my thoughts (the text is "under-construction" and liable to change quickly).''} [P70]\\\\
    \textit{``Worrying about complete sentences and grammar while brainstorming would slow things down considerably ... but necessary for a final release.''} [P227]\\\\
    \textit{``Initial document writing is mainly non-collaborative, whereas later it's a matter of tweaking and improving with the feedback of others.''} [P178]
\end{myquote}
Later stages, on the other hand, are described as the time when most of the content has been added to the document and the writers can now focus on improving different aspects of the document during Reviewing and Copy-Editing phases.

\begin{myquote}{0.2in}
    \textit{``Document creation and document perfection are fundamentally different.  In my opinion, the best way to create a collaborative document is to get a rough draft made as quickly and dirtily as possible and then begin to improve it; different forms of assistance are required for each scenario.''} [P237]\\
\end{myquote}
These later stage activities are identified as Proofreading e.g. proofing and formatting, Task Management (e.g. addressing pending comments or TODO items), Collaborative Activities such as adding collaborators, communicating with collaborators through comments and change tracking functionalities, etc. as well as Reviewing and Finalizing activities including fact checking, adding references, setting required permissions, etc.

\begin{myquote}{0.2in}
    \textit{``When getting started, Outline or Structure help is needed Later on in the process, Editing, fact checking, adding references type of help is needed ''} [P84]\\\\
    \textit{``[In later stages] 1. Update me of unaddressed/unread comments that I should follow up on. 2. Help me identify similar comment available in other documents that I can use for reference.''} [P37]\\\\
    \textit{``At the drafting stage, making sure the document is structured properly and all the bases are covered is paramount. At later stages, getting feedback and sign-off become much more important. It'd be great to more easily track changes.''} [P154]\\\\
    \textit{``At the end of the writing process it is helpful to have a spelling and grammar check, with perhaps some suggestions on structure, yet I find suggestion DURING writing to be distracting.''} [P182] \\\\
    \textit{``At the beginning providing table contents, title formats, and captioning. Later can add references, etc.''} [P194]\\
\end{myquote}

An interesting quality of later stages is that the document is known to be more ``mature'' with most of the content already included and structured. This quality has at least two different implications for what support can and should be provided at earlier versus later stages of writing. First, since in later stages the structure and the content of the document is highly stable the system can provide more end to end and global feedback as opposed to suggestions that are relevant to a specific part of the text only (e.g. identifying missing topics to be included versus spelling errors to be fixed). Second, with more content in place and a longer history of edits, intelligent writing assistants can be more reliable in predicting what support is needed.  

\begin{myquote}{0.2in}
    \textit{``When I'm actively working on creating the document I want suggestions around better writing style, but focused on what I'm doing at that moment.  Once the document is more mature I'd want feedback on the end to end document, not a specific word here or there.''} [P106]\\\\
    \textit{``During the draft phase, there will be a lot of changes that just won't stick. At reviewing phase it would be helpful to objectively view the whole document to suggest improvements.''} [P207]\\\\
    \textit{``Once a lot of content is in a document, a `bot' may be able to warn that you are going to change something that was just edited.''} [P77]\\\\
    \textit{``Intelligence should improve as the document matures.  The intent of the document, the subject matter, and the style of the document will become more clear as it evolves.''} [P78]
\end{myquote}

%The main takeaways from what was discussed can be summarized as three implications for design:
The following three design implications are our main takeaway from the preceding analysis:
\begin{enumerate}
    \item Intelligent Support should be provided based on the activities that are pertaining to the current stage of document evolution (i.e. early versus later stages).% in order to be appreciated by the writers.
    \item Writers are in a focused mode during earlier stage of writing and the interruptions by the system should be minimized. 
    \item Users can benefit from a higher level of control over the writing process in earlier stages with outlining, structuring or searching functionalities that are provided on demand. During later stages intelligent systems can be more proactive in providing feedback and suggestions to improve the overall document quality.
\end{enumerate}

\subsection{Supporting Different Phases of Writing}
According to Lowry et al's Taxonomy of Writing Activities \cite{lowry2004}, writers are known to go through different phases throughout the writing process. These phases are characterized as brainstorming, outlining, drafting, reviewing, revising and copy editing. This view of writing activities is largely inline with Flower and Hayes model that specifies planning, translating and reviewing as three main processes involved.

A qualitative analysis of our participants' responses reveals that the idea of going through different phases of writing during the process of writing documents resonates with them. They describe these phases in a variety of terms:
\textit{``from document creation to document perfection''} [P237], \textit{``starting from nothing phase''} [P98], \textit{``Rough draft vs final draft''} [P?], \textit{``Draft, Editing, Polishing''} [P?, P220], \textit{``Creative or Brainstorming, `culling the first main draft', draft editing, reviewing, finalizing''} [P?] \textit{``Outlining, Writing, Consulting''} [P158], \textit{``Schedule (content requirements), Reminders \& goals, Refresh''} [P135], \textit{``early drafting, end of drafting, reviewing''} [P224] etc.

%Similar to the theme described in the previous subsection those participants who resonated with these phases of writing
Participants described groups of activities that are associated with each phase and hence could use targeted support during that phase.

\begin{myquote}{0.2in}
    \textit{``There are appropriate tasks for every phase that might not apply for all others and assistance in remembering them would be great. Like assistance for spellcheck/alignment  is much better suited to the end of \textbf{drafting}. Reminders to share or tag people are better suited for \textbf{reviewing}.''} [P224]\\\\
    \textit{``Different stages require different approaches: \textbf{drafting} is a ``throw in all ideas'', but \textbf{finalizing} is ``polish wording and structure''.  E.g.: Worrying about complete sentences and grammar while brainstorming would slow things down considerably … but necessary for a final release.''} [P227]\\\\
    \textit{``\textbf{Brainstorming} vs. \textbf{Authoring} vs. \textbf{Finalizing} have very different needs.''} [P138]\\\\
    \textit{``Writing stages differ: \textbf{Creative or brainstorming}. Culling the main \textbf{first draft}. \textbf{Draft editing} and \textbf{review}. \textbf{Finalization} of the document. Each involves a different skill set.''} [P113]\\\\
    \textit{``\textbf{Outlining} should help you structure your document before you begin.  \textbf{Writing} should check for spelling and grammar.  \textbf{Consulting} should make sure information is accurate.''} [P158]\\\\
    \textit{``The assistant could provide different services at different stages of the doc, such as during \textbf{editing} would provide with content suggestions; while \textbf{reviewing} it could provide with hints to include the right audience; on \textbf{publishing} it could help with Permission settings and privacy/compliance reviews; etc ...''} [P50]
\end{myquote}

%The common theme among this group of participants was that (1) writers do go through multiple phases during the writing process and (2) different phases involve different activities and hence require different skills and type of support.

\begin{myquote}{0.2in}
    \textit{``Designing a structure of a document and inviting/assigning contributors is different than editing/revising drafts.''} [P24]\\\\
    \textit{``the feedback required is different at each stage.''} [P118]
\end{myquote}

A second round of qualitative coding of these responses resulted in identifying different activities that are associated with different phases of writing as perceived by our participants:
\begin{itemize}
    \item \emph{\textbf{Planning/Brainstorming Phase:}} Outlining/Diagramming [P36], section naming and setup [P46], help with structuring the document [P158]
    \item \emph{\textbf{Drafting Phase:}} Getting content or wording help [P44], structuring support to offload the mind [P63], support for sharing [P167]
    \item \emph{\textbf{Reviewing / Consulting Phase:}} notifications for formatting, grammar and spelling errors [P40], look of the document [P12], proofing [P75, P224], repetitive language usage [P167], highlighting unaddressed comments [P37], hints to include the right audience [P50, P133, P167], reminders to share or tag people [P224], fact checking [P123, P158], adding required references and sources [P133]
    \item \emph{\textbf{Finalizing / Publishing Phase:}} checking for broken paragraphs or tables before printing [P42], help with permission settings [P50], help with requesting required privacy and compliance reviews
\end{itemize}

In summary, writers recognize multiple phases during the writing process, they use a wide range of terminology to refer to them which can be grouped and mapped (at a high level) to the taxonomy of writing activities by Lowry et al \cite{lowry2004}. Similar to the previous theme of early versus late stages of document's evolution, different phases of writing are affiliated with different activities and the type of support should be tailored to the current phase of writing.
Finally, while these phases of writing can be seen as individual authors' mental state and hence are more complex to detect than early versus later stages of document evolution (as discussed in the previous subsection), we can see an overarching time-based ordering to these phases starting from brainstorming and outlining, moving to drafting, reviewing and finalizing.

%Please note that while there is no clear separation between these phases (e.g. end of outlining and early drafting, late drafting versus reviewing, etc), our participants do associate some phases to earlier stages of document evolution and other phases to the later stages.

\subsection{Supporting Different Writers' Intents}
Writing documents usually spans over multiple sessions of activity that are distributed over the lifetime of that document. 
When a writer attends to a document (representing the workspace), to do a particular task, they bring with them a general understanding of the current stage of a document (more clearly visible in SAW scenarios) and a basic idea of what to look for or what activity to do (see also Gutwin and Greenberg's \cite{gutwin2002} descriptive framework of workspace awareness for real-time groupware).

%A relevant theme to ``phases of writing'' is the intent of the writer who comes to a document at different stages during its lifetime.

%Similar to what Gutwin and Greenberg \cite{gutwin2002} describe in their descriptive framework of workspace awareness for real-time groupware, when a writer attends to a document (representing the workspace), to do a particular task, they bring with them a general understanding of the current stage of a document (more clearly visible in SAW scenarios) and a basic idea of what to look for or what activity to do.

%A common theme across a group of our participants was their intent or goal of attending to a document. They 
Our participants referred to different goals they have when they attend to a document at different times, and that based on this goal they are seeking different types of support from the system.

\begin{myquote}{0.2in}
    \textit{``Sometimes I'm just scanning a document for minor edits and other times I'm going full bore and ignoring small mistakes.''} [P15]\\\\
    \textit{``[when] writing [I'm] less focused on actual facts, where as reviewing will need to be very factual.''} [P123]\\\\
    \textit{``Sometimes you just need to get thoughts onto "paper" and other times you need to review feedback, clean up the content and get ready to publish.''} [P147]\\\\
\end{myquote}

%We note that the awareness of the writer's intent at the time they are attending to the document is already reflected in the writer's mental state in single author scenarios and the system can support this state by providing support that matches the intended activity.
A system can provide support that matches the intended activity: For example, hiding comments and change tracking annotations when the user is not in ``review mode'' or disabling editing when the user is in ``reading mode'' can help simplify the user's interaction with the writing environment and minimize changes by accident.

However, once we move to multi-author scenarios there is a need for a shared awareness of the document as the workspace, and the intent of a collaborator is impacted by this awareness.

\begin{myquote}{0.2in}
    \textit{``An ideal collaborative writing environment would allow users the choice of whether collaborators can view only or make edits to a document because the document should not be editable in certain situations.''} [P206]
\end{myquote}

%The final theme that was derived from our qualitative analysis is regarding the awareness of the stage that the shared document currently is and is predominantly visible in Collaborative Writing scenarios. The next subsection elaborates on this theme.

\subsection{Awareness of Document's Stage}
So far the three themes discussed above highlighted the importance of the detection of the current stage of a document or its corresponding writing phases to be able to provide writing support that is tailored to this stage. A distinct and interesting theme that was discovered through the qualitative coding of our survey responses was that the awareness of the stage of document's evolution is not only crucial for the system, i.e. an intelligent writing assistant, but is also crucial for collaborating authors who join a shared document at different stages of its lifetime. 

To clarify, while in single author scenarios a writer who attends to a document at some point in time generally has a good understanding of the current stage of a document and what the next steps should be, in collaborative writing scenarios developing and maintaining the workspace awareness is challenging \cite{gutwin2002}.

%In unpacking some of our participants responses we noticed a desire for a shared awareness of the document when multiple authors are involved. 

\begin{myquote}{0.2in}
    \textit{`` ...  At the end I need to know who all has access, if any feedback has been left, what stage the doc is in (in review, in implementation, locked, stale, etc.).''} [P81]\\\\
    \textit{``The requirements from collaboration will vary over the lifespan of the document from creation to delivery to retirement.''} [P80]\\\\
\end{myquote}

Gutwin and Greenberg \cite{gutwin2002} motivate the importance of workplace awareness for collaborative scenarios which can reduce effort, increase efficiency and reduce errors for the activities of collaboration.
%For example, awareness of the stage of document helps with coordination of and suggesting the ways new collaborators can contribute and assist the writing process.

Assisting others with their local tasks is an integral part of collaboration and one that also benefits from workspace awareness. Awareness in this situation is useful because it helps people determine what assistance is \textit{required} and what is \textit{appropriate}. This was confirmed by our participants:

%Our participants articulated that awareness of what stage the document is currently in can greatly help with anticipating what assistance is expected and appreciated by other collaborators.

\begin{myquote}{0.2in}
    \textit{``From the previous experiences, we tend to give more feedback in the beginning than the later when the content is mostly completed.''} [P195]
\end{myquote}

Some of our participants were proactive in suggesting ways that an intelligent system can detect the current stage of a document and share that information with other collaborators who attend the document at different times.

\begin{myquote}{0.2in}
    \textit{``[The system can track] the number of people with the document opened for edit.  Tracking the "shares" of the document to know when it's sent for review or edit. the intelligent assistant that provided me the prompts to share it for review or editing would know [the stage of the document] from the selections I make.''} [P172]
\end{myquote}

\subsection{Summary of Findings}
Our survey data provided different insights regarding how writers perceive the stages of a document evolution and what types of writing assistance is expected at these stages of document authoring.

The qualitative analysis of survey responses indicated that the writers in our population perceive a document stage in three different yet related ways: (1) temporal stages of document evolution; (2) phases of writing and (3) modes of writing. 

Given the complexity of the writing process and how different cognitive sub-processes of planning, translating and reviewing interact, we are yet to explore automatic methods that can detect these writing phases \cite{baaijen2012, leijten2013, conijn2019}.
However, our qualitative findings highlight an overarching temporal ordering of these writing phases and modes of writing as reflected in the mental model of our participants.
%that could be used as a first step towards characterizing stages of document authoring.

Further, our qualitative findings indicate that awareness of a current document's stage of evolution has implications for both users and the system.
While intelligent writing assistants can use this information to provide writing assistance to writers that is tailored to the current stage of the document, in collaborative scenarios, new collaborators who join a shared document at different points throughout the document's lifetime can better coordinate their next actions such that in can assist others by contributing to the current stage of writing. 

In the next section we revisit the notion of temporal stages of document evolution through a different lens, by characterizing differences in the users' interaction logs of a commercial writing application. Our main goal with this quantitative analysis is to verify our qualitative findings at scale and through a record of actual users interactions as they are writing documents.


==> sec.SupportingWriting.tex <==
\section{Writing at the Workplace} 
Most research on the writing process has been carried out in the context of education. Thus, little focus has been put on the particularities which arise when the writing process is carried out by information workers who need to write documents as a part of their daily routine at the workplace.

There are many open questions in this space including how common writing documents at the workplace is, what support is needed, what are the expectations of an intelligent writing tool and whether there is a need for tailored support at different stages of writing?

To address these questions, we conducted a survey at a large technology company with a range of close-ended as well as open-ended questions. The survey data helped
us understand how document writing is currently done by enterprise workers, how commonly it is done and what support is currently needed that is not provided by popular writing tools.

\subsection{Survey}
We distributed a survey to multiple mailing lists within this company and collected 175 responses (completion rate: 70\%). 

Our survey started with a section on demographics including Job roles, number of current projects, team size, etc. The next section involved different questions regarding writing documents at the workplace which helped us verify whether writing documents at the workplace is a common practice, What tools are frequently used for writing documents and how often these documents involve other collaborators as well.

Respondents came from a diverse set of roles ranging from product managers and software developers to sales people and administrative assistants.  Multi-tasking on different projects was a common trend among them, with 75\% working on at least 3 projects and the majority have been working at this company for more than 5 years (63\%).
% \item {\verb|anonymous,review|}: Suitable for a ``double-blind''

%\begin{verbatim}
%\documentclass[sigconf,authordraft]{acmart}
%\end{verbatim}

\subsection{Main Findings}
Our survey data confirmed that writing documents is very common at the workplace. 87\% of our respondents mentioned they do need to write documents as a part of their work routine. They use a wide range of writing tools including Microsoft Word Desktop Client (89\%) and Online Client (49\%), followed by Notepad / Notepad++ (19.3\%), OneNote (16\%), Overleaf / Sharelatex (11.1\%), Google Docs (8.2\%), etc.

Collaboration on these documents was also a common theme among our participants with the majority (74\%) collaborating on at least 25\% of their documents.

As a first step towards understanding whether or not there is a need for different types of support at different stages of document evolution, the next segment of our survey included a series of questions to gauge real users perceptions and attitudes towards this concept. More formally, the participants were asked \textit{``Should an intelligent writing assistant provide different types of support at different stages of writing in the document?''} with a binary Yes / No response type.

Over 70\% of our participants expressed a need for different types of support at different stages of writing by answering Yes to this question. The follow up open-ended questions to elaborate on their rationales for their response to this initial question revealed how these stages are perceived by the participants and that what support is needed at these stages. 

The responses to these questions
were all analyzed using affinity diagramming. Data was initially clustered using open coding producing
19 clusters. Clusters were then analyzed using axial coding to identify overall themes in the data. We found that saturation for our
qualitative data occurred approximately after 80 participants, no
new clusters of information were identified. However, we continued
to cluster these responses for the remaining participants, particularly
attuned to data that might expand our clusters or add nuance to
our analysis. These clusters resulted in five broad themes, namely:
(1) The need for tailored support in different stages is associated with both \mg{have we introduced these acronyms at this point?} SAW and CW scenarios; (2) Supporting Early versus Later Stages of Document Evolution; (3) Supporting different phases of writing; (4) Supporting different modes or intents of writing; and (5) Awareness of Stage of Document is essential both for the intelligent System and the collaborating writers. We describe more details about these themes in the following subsections.

\subsection{Stage-based Support for both SAW and CW}
%Writers require different support at different stages of writing both in SAW and CW scenarios.

Single author Writing (SAW) is defined as writing conducted by one individual that involves planning, drafting and reviewing (Lowry et al., 2004)
Collaborative Writing (CW) builds on single-author writing by involving multiple people, thus increasing the complexity of the writing process (Galegher and Kraut, 1994).

While the complexity of CW scenarios are generally more amplified relative to SAW scenarios, a qualitative analysis of these survey responses indicated that the need for a tailored support at different stages of writing is not the case for CW settings only. While some of the participants talked about multi-author scenarios, the majority of responses could be applied to either of these scenarios. 
\begin{quote}
\textit{``in and ideal scenario I would just do some sort of content dump to the system and the system structures this text. So that I don't have to think about paragraphs, sections, where to put what etc. And then in later stages I want help with how to nicely formulate things. That's not only in a collaborative setting though.''} [P10]
\end{quote}

In unpacking the quote above we also see a time-based notion of stages of document writing that is further discussed in the following subsection.

\subsection{Supporting Early versus Late Stages of Document}
The Stages Model of Writing (Rohman, 1965) focuses on the evolution of the text as an external by-product of the writing where the main three stages of pre-writing, writing and rewriting are separated in time. While the more recent models (e.g. Flower and Hayes (1984)) argue that a more realistic model of writing needs to focus on the mental processes involved in the writing process and that these mental processes are interleaved, hierarchically embedded and are not executed in a linear order, these models are indeed complementary and are not in conflict (Mitchell, 1996). 

In fact, once we shift our view to the document as the by product of this process we can see some time based ordering of these high level stages of document evolution. 

This view was shared amongst many of our participants who referred to these stages as early versus later stages of document writing.

The early stages of writing was perceived to be a highly focused writing mode and many participants expressed a desire for fewer interruptions and more specifically fewer system's suggestions and notifications for minor fixes and improvements. 
\begin{quote}
\textit{``I want fewer interruptions when i am focusing on adding content early in the document writing process.''} [P11]\\\\
\textit{``As someone who primarily writes documents in LaTeX, I like the ability to focus on writing the content without having to worry about formatting. Then only once the content is put down do I go back and tweak the look of the document. This allows me to focus on different aspects of the documents at different stages.''} [P12]\\\\
\textit{``Notifying me of grammar and spelling errors when I'm trying to get my thoughts out is really just a distraction. I prefer when these suggestions are made at a later editing stage.''} [P40]
\end{quote}\\
The qualitative analysis of these responses indicated that participants can associate different phases of writing including Planning, Outlining and Early Drafting to \textit{Early Stages of Writing}. 

As well, a variety of activities that are pertaining to earlier stages of writing were discussed which revealed the types of support that are the most appreciated in these early stages. Among them, outlining and deciding on the structure of the document as well as searching for relevant content to cover were perceived as early stage activities. 
\begin{quote}
    \textit{``Brainstorming and scope defining support \textbf{early on} that helps develop a basic outline and framework. It would be great for a writing assistant to help with the `starting from nothing' phase.''} [P98]\\\\
    \textit{``The needs at different stages may be very different. E.g. for structural changes, they better take place as \textbf{early} as possible; while for minor fixes or suggestions, they can come \textbf{later} when the body of text is by and large stable.''} [P64]\\\\
    \textit{``When \textbf{getting started}, Outline or Structure help is needed; \textbf{Later on} in the process, Editing, fact checking, adding references type of help is needed.''} [P84]\\\\
    \textit{``\textbf{Early:} Focus and scope - needed at the beginning to understand what to write about and how much; this is often org dependent and the ability to create org-specific templates and help advice would be amazing.  \textbf{Mid:} Content analysis and comparison, to highlight style and completeness differences in different areas.  \textbf{Late:} Advice on structural features and cleanups that can save time and improve accessibility.''} [P219]\\\\
    \textit{``Would be great to enter some notes and have an outline constructed. \textbf{Later} it would be great to have research done for me if I need a supporting quote or need a chart from another document. \textbf{Finally} it would help to have suggestions for alternatives to overused words.''} [P57]
\end{quote}\\
Similarly, variety of activities that are not crucial to earlier stages of writing were described for them system support can be perceived as \textit{distracting}, \textit{annoying} or \textit{not necessary}.
Overall, minor fixes, proofing and grammar fixes, collaborative activities such as commenting and change tracking are perceived as not helpful nor appreciated during early stages of document evolution.
\begin{quote}
    \textit{``Different actions and needs are required for each stage of writing; i.e. there is no need to suggest spacing and layout changes when I've just started writing down my thoughts (the text is "under-construction" and liable to change quickly).''} [P70]\\\\
    \textit{``Worrying about complete sentences and grammar while brainstorming would slow things down considerably ... but necessary for a final release.''} [P227]\\\\
    \textit{``Initial document writing is mainly non-collaborative, whereas later it's a matter of tweaking and improving with the feedback of others.''} [P178]
\end{quote}\\
Later stages, on the other hand, are described as the time that most of content is added to the document and the writers can now focus on improving different aspects of the document during Reviewing and Copy-Editing phases.

\begin{quote}
    \textit{``Document creation and document perfection are fundamentally different.  In my opinion, the best way to create a collaborative document is to get a rough draft made as quickly and dirtily as possible and then begin to improve it; different forms of assistance are required for each scenario.''} [P237]\\
\end{quote}\\
These later stage activities are identified as Proofreading e.g. proofing and formatting, Task Management (e.g. addressing pending comments or TODO items), Collaborative Activities such as adding collaborators, communicating with collaborators through comments and change tracking functionalities, etc as well as  Reviewing and Finalizing activities including fact checking, adding references, setting required permissions, etc.

\begin{quote}
    \textit{``When getting started, Outline or Structure help is needed Later on in the process, Editing, fact checking, adding references type of help is needed ''} [P84]\\\\
    \textit{``[In later stages] 1. Update me of unaddressed/unread comments that I should follow up on. 2. Help me identify similar comment available in other documents that I can use for reference.''} [P37]\\\\
    \textit{``At the drafting stage, making sure the document is structured properly and all the bases are covered is paramount. At later stages, getting feedback and sign-off become much more important. It'd be great to more easily track changes.''} [P154]\\\\
    \textit{``At the end of the writing process it is helpful to have a spelling and grammar check, with perhaps some suggestions on structure, yet I find suggestion DURING writing to be distracting.''} [P182] \\\\
    \textit{``At the beginning providing table contents, title formats, and captioning. Later can add references, etc.''} [P194]\\
\end{quote}

An interesting quality of later stages is that the document is known to be more ``mature'' with most of the content already included and structured. This quality has at least two different implications for what support can be and should be provided at earlier versus later stages of writing. First, since in later stages the structure and the content of the document is highly stable the system can provide more end to end and global feedback as opposed to suggestions that are relevant to a specific part of text only (e.g. identifying missing topics to be included versus spelling errors to be fixed). Second, with a larger volume of content in place and a longer history of edits intelligent writing assistants can be more reliable in predicting what support is needed.  

\begin{quote}
    \textit{``When I'm actively working on creating the document I want suggestions around better writing style, but focused on what I'm doing at that moment.  Once the document is more mature I'd want feedback on the end to end document, not a specific word here or there.''} [P106]\\\\
    \textit{``During the draft phase, there will be a lot of changes that just won't stick. At reviewing phase it would be helpful to objectively view the whole document to suggest improvements.''} [P207]\\\\
    \textit{``Once a lot of content is in a document, a `bot' may be able to warn that you are going to change something that was just edited.''} [P77]\\\\
    \textit{``Intelligence should improve as the document matures.  The intent of the document, the subject matter, and the style of the document will become more clear as it evolves.''} [P78]
\end{quote}\\

The main takeaways from what was discussed can be summarized as three implications for design:
\begin{enumerate}
    \item Intelligent Support should be provided based on the activities that are pertaining to the current stage of document evolution (i.e. early versus later stages) in order to be appreciated by the writers.
    \item Writers are in a focused mode during earlier stage of writing and the interruptions by the system should be minimized. 
    \item Users can benefit from a higher level of control over the writing process in earlier stages with outlining, structuring or searching functionalities that are provided on demand. During later stages intelligent systems can be more proactive in providing feedback and suggestions to improve the overall document's quality.
\end{enumerate}
\subsection{Supporting Different Phases of Writing}
Referencing Lowry et al (2004) Taxonomy of Writing Activities, writers are known to go through different phases throughout the writing process. These phases are characterized as brainstorming, outlining, drafting, reviewing, revising and copy editing. This view of writing activities is largely inline with Flower and Hayes model that specifies planning, translating and reviewing as three main processes involved.

A qualitative analysis of our participants responses reveals that authors (in our population) do resonate with different phases of writing that they go through during the process of writing documents. They describe these phases in a variety of terms to distinguish them from one another:
\textit{``from document creation to document perfection''} [P237], \textit{``starting from nothing phase''} [P98], \textit{``Rough draft vs final draft''} [P?], \textit{``Draft, Editing, Polishing''} [P?, P220], \textit{``Creative or Brainstorming, `culling the first main draft', draft editing, reviewing, finalizing''} [P?] \textit{``Outlining, Writing, Consulting''} [P158], \textit{``Schedule (content requirements), Reminders \& goals, Refresh''} [P135], \textit{``early drafting, end of drafting, reviewing''} [P224] etc.

Similar to the theme described in the previous subsection those participants who resonated with these phases of writing described groups of activities that are associated with each phase and hence needs support while the writer is in that phase of writing.

\begin{quote}
    \textit{``There are appropriate tasks for every phase that might not apply for all others and assistance in remembering them would be great. Like assistance for spellcheck/alignment  is much better suited to the end of \textbf{drafting}. Reminders to share or tag people are better suited for \textbf{reviewing}.''} [P224]\\\\
    \textit{``Different stages require different approaches: \textbf{drafting} is a ``throw in all ideas'', but \textbf{finalizing} is ``polish wording and structure''.  E.g.: Worrying about complete sentences and grammar while brainstorming would slow things down considerably … but necessary for a final release.''} [P227]\\\\
    \textit{``\textbf{Brainstorming} vs. \textbf{Authoring} vs. \textbf{Finalizing} have very different needs.''} [P138]\\\\
    \textit{``Writing stages differ: \textbf{Creative or brainstorming}. Culling the main \textbf{first draft}. \textbf{Draft editing} and \textbf{review}. \textbf{Finalization} of the document. Each involves a different skill set.''} [P113]\\\\
    \textit{``\textbf{Outlining} should help you structure your document before you begin.  \textbf{Writing} should check for spelling and grammar.  \textbf{Consulting} should make sure information is accurate.''} [P158]\\\\
    \textit{``The assistant could provide different services at different stages of the doc, such as during \textbf{editing} would provide with content suggestions; while \textbf{reviewing} it could provide with hints to include the right audience; on \textbf{publishing} it could help with Permission settings and privacy/compliance reviews; etc ...''} [P50]
\end{quote}

The common theme among this group of participants was that (1) writers do go through multiple phases during the writing process and (2) different phases involve different activities and hence require different skills and type of support.

\begin{quote}
    \textit{``Designing a structure of a document and inviting/assigning contributors is different than editing/revising drafts.''} [P24]\\\\
    \textit{``the feedback required is different at each stage.''} [P118]
\end{quote}

A second round of qualitative coding of these responses resulted in identifying different activities that are associated with different phases of writing as perceived by our participants.\\\\ 
\noindent \emph{\textbf{Planning / Brainstorming Phase:}}
\begin{itemize}
    \item Outlining / Diagramming [P36]
    \item Sections naming and setup [P46]
    \item help with structuring the document [P158]
\end{itemize}

\noindent \emph{\textbf{Drafting Phase:}}
\begin{itemize}
    \item Getting content or wording help [P44]
    \item Structuring support to offload the mind [P63]
    \item Sharing support [P167]
\end{itemize}

\noindent \emph{\textbf{Reviewing / Consulting Phase:}}
\begin{itemize}
    \item notifications for formatting, grammar and spelling errors [P40]
    \item look of the document [P12]
    \item proofing [P75, P224]
    \item repetitive language usage [P167]
    \item highlighting unaddressed comments [P37]
    \item hints to include the right audience [P50, P133, P167]
    \item reminders to share or tag people [P224]
    \item fact checking [P123, P158]
    \item adding required references and sources [P133]
\end{itemize}

\noindent \emph{\textbf{Finalizing / Publishing Phase:}}
\begin{itemize}
    \item checking for broken paragraphs or tables before printing [P42]
    \item help with permission settings [P50]
    \item help with requesting required privacy and compliance reviews
\end{itemize}

To conclude this theme, writers recognize multiple phases during the writing process, they use a wide range of terminology to refer to them which can be grouped and mapped (at a high level) to the taxonomy of writing activities by Lowry et al (2004). As well, similar to the previous theme of early versus late stages of document's evolution, different phases of writing are affiliated with different activities and the type of support should be tailored to the current phase of writing.
Finally, while these phases of writing can be seen as individual authors' mental state and hence are more complex to detect than early versus later stages of document evolution (as discussed in the previous subsection), while unpacking the way our participants described these phases we can see an overarching time-based ordering to these phases starting from brainstorming and outlining, moving to drafting, reviewing and finalizing.

Please note that while there is no clear separation between these phases (e.g. end of outlining and early drafting, late drafting versus reviewing, etc), our participants do associate some phases to earlier stages of document evolution and other phases to the later stages.

\subsection{Supporting Different Writers' Intents}
A relevant theme to ``phases of writing'' is the intent of the writer who comes to a document at different stages during its lifetime.

Writing documents usually spans over multiple sessions of activity that are distributed over the lifetime of that document. 

Similar to what Gutwin and Greenberg (2002) describe in their descriptive framework of workspace awareness for real-time groupware, when a writer attends to a document (representing the workspace), to do a particular task, they bring with them a general understanding of the current stage of a document (more clearly visible in SAW scenarios) and a basic idea of what to look for or what activity to do.

A common theme across a group of our participants was their intent or goal of attending to a document. They referred to different goals they have when they attend to a document they are working on at different times of attending to the document, and that based on this goal they are seeking different types of support from the system.

\begin{quote}
    \textit{``Sometimes I'm just scanning a document for minor edits and other times I'm going full bore and ignoring small mistakes.''} [P15]\\\\
    \textit{``[when] writing [I'm] less focused on actual facts, where as reviewing will need to be very factual.''} [P123]\\\\
    \textit{``Sometimes you just need to get thoughts onto "paper" and other times you need to review feedback, clean up the content and get ready to publish.''} [P147]\\\\
\end{quote}

We note that the awareness of the writer's intent at the time they are attending to the document is already reflected in the writer's mental state in single author scenarios and the system can support this state by providing support that matches the intended activity.
For example, hiding comments and change tracking annotations when the user is not in ``review mode'' or disabling editing when the user is in ``reading mode'' can help simplify the user's interaction with the writing environment and minimize changes by accident.

However, once we move to multi-author scenarios there is a need for a shared awareness of the document as the workspace and the intent of a collaborator is impacted by this awareness.

\begin{quote}
    \textit{``An ideal collaborative writing environment would allow users the choice of whether collaborators can view only or make edits to a document because the document should not be editable in certain situations.''} [P206]
\end{quote}

The final theme that was derived from our qualitative analysis is regarding the awareness of the stage that the shared document currently is and is predominantly visible in Collaborative Writing scenarios. The next subsection elaborates on this theme.

\subsection{Awareness of Document's Stage}
So far the three themes discussed above highlighted the importance of the detection of the current stage of a document or its corresponding writing phases for an intelligent system to be able to provide writing support that is tailored to this stage. A distinct and interesting theme that was discovered through the qualitative coding of our survey responses was that the awareness of the stage of document's evolution is not only crucial for the system, i.e. an intelligent writing assistant, but is also crucial for collaborating authors who join a shared document at different stages of its lifetime. 

To clarify, while in single author scenarios a writer who attends to a document at some point in time generally has a good understanding of the current stage of a document and what the next steps should be, in collaborative writing scenarios developing and maintaining the workspace awareness is shown to be challenging (Gutwin and Greenberg (2002)).

In unpacking some of our participants responses we noticed a desire for a shared awareness of the document when multiple authors are involved. 

\begin{quote}
    \textit{`` ...  At the end I need to know who all has access, if any feedback has been left, what stage the doc is in (in review, in implementation, locked, stale, etc.).''} [P81]\\\\
    \textit{``The requirements from collaboration will vary over the lifespan of the document from creation to delivery to retirement.''} [P80]\\\\
\end{quote}

Gutwin and Greenberg (2002) motivate the importance of workplace awareness for collaborative scenarios which can reduce effort, increase efficiency and reduce errors for the activities of collaboration.
For example, awareness of the stage of document helps with coordination of and suggesting the ways new collaborators can contribute and assist the writing process.

Assisting others with their local tasks is an integral part of collaboration and one that also benefits from workspace awareness. Awareness in this situation is useful because it helps people determine what assistance is \textit{required} and what is \textit{appropriate}.

As articulated by our participants awareness of what stage the document is currently in can greatly help with anticipating what assistance is expected and appreciated by other collaborators.

\begin{quote}
    \textit{``From the previous experiences, we tend to give more feedback in the beginning than the later when the content is mostly completed.''} [P195]
\end{quote}

Some of our participants were proactive in suggesting ways that an intelligent system can detect the current stage of a document and share that information with other collaborators who attend the document at different times.

\begin{quote}
    \textit{``[The system can track] the number of people with the document opened for edit.  Tracking the "shares" of the document to know when it's sent for review or edit. the intelligent assistant that provided me the prompts to share it for review or editing would know [the stage of the document] from the selections I make.''} [P172]
\end{quote}


